A Fast, Accurate and Oscillation-free Spectral Collocation Solver for High-dimensional Transport Problems

Transport phenomena-describing the movement of particles, energy, or other physical quantities-are fundamental in various scientific disciplines, including nuclear physics, plasma physics, astrophysics, engineering, and the natural sciences. However, solving the associated seven-dimensional transport equations poses a significant computational challenge due to the curse of dimensionality. We introduce the Tensor Train Superconsistent Spectral (T${^2}$S${^2}$) solver to address this challenge, integrating Spectral Collocation for exponential convergence, Superconsistency for stabilization in transport-dominated regimes, and Tensor Train format for substantial data compression. T${^2}$S${^2}$ enforces a dimension-wise superconsistent condition compatible with tensor structures, achieving extremely low compression ratios, in the order of $(10^{-12})$, while preserving spectral accuracy. Numerical experiments on linear problems demonstrate that T${^2}$S${^2}$ can solve high-dimensional transport problems in minutes on standard hardware, making previously intractable problems computationally feasible. This advancement opens new avenues for efficiently and accurately modeling complex transport phenomena.

==> abstract-all-versions.tex <==
%%(149 words)
\begin{comment}
Transport phenomena are fundamental in nuclear and plasma physics,
natural sciences, and engineering. Solving the associated
high-dimensional advection-diffusion-reaction equations, however,
presents a significant computational challenge.  We introduce the
Tensor Train Superconsistent Spectral (\mymethod{}) solver, a novel
approach enabling fast, accurate, and stable solutions in
six-plus-time dimensions. \mymethod{} leverages Spectral Collocation
for exponential convergence, Superconsistency for stabilization, and
the Tensor Train format for extreme data compression. By enforcing a
suitable dimension-wise superconsistent condition compatible with
tensor structures, \mymethod{} achieves compression ratios of
$\mathcal{O}(10^{-12})$ while preserving spectral accuracy.  Numerical
experiments demonstrate that \mymethod{} can solve such
high-dimensional transport problems in minutes on standard computing
hardware.  Using traditional methods, these tasks would require
millions of years on modern supercomputers. This proposed method makes
previously intractable high-dimensional problems in transport physics
and engineering computationally accessible.
\end{comment}

\begin{comment}
Transport phenomena are fundamental in nuclear and plasma physics,
natural sciences, and engineering. However, solving the associated
high-dimensional advection-diffusion-reaction equations remains a
major computational challenge. We introduce the Tensor Train
Superconsistent Spectral (\mymethod{}) solver, a novel approach that
enables fast, accurate and stable solutions in six-plus-time
dimensions. \mymethod{} builds on Spectral Collocation for exponential
convergence, Superconsistency for stabilization, and the Tensor Train
format for extreme data compression.  By enforcing a suitable
dimension-wise superconsistent condition compatible with tensor
structures, \mymethod{} achieves compression ratios of
$\mathcal{O}(10^{-12})$ while maintaining spectral accuracy.  The
numerical experiments demonstrate that
\mymethod can solve six-plus-time dimensional transport problems 
in minutes on standard computing hardware. Using traditional methods, the same
tasks would require millions of years on 
modern supercomputers. 
The proposed method makes previously 
intractable high-dimensional problems in transport physics and engineering 
computationally accessible.
\end{comment}

\begin{comment}
%% 150 words
Transport phenomena play a fundamental role in nuclear and plasma
physics, natural sciences, and engineering, yet solving the associated
high-dimensional advection-diffusion-reaction equations remains a
major computational challenge. We introduce the Tensor Train
Superconsistent Spectral (\mymethod{}) solver, a novel approach that
enables fast, accurate and stable solutions to these equations in
six-plus-time dimensions. \mymethod{} integrates Spectral Collocation
for exponential convergence, Superconsistency for unconditional
stability, and the Tensor Train format for extreme data
compression. By enforcing a dimension-wise Superconsistent condition
compatible with tensor structures, \mymethod{} achieves compression
ratios of $\mathcal{O}(10^{-12})$while maintaining spectral
accuracy. Our numerical experiments demonstrate that \mymethod{} can
solve six-plus-time dimensional transport problems in minutes on
standard computing hardware—tasks that would require millions of years
on current supercomputers using traditional methods. \mymethod{}
solver makes previously intractable high-dimensional problems in
transport physics and engineering computationally feasible.
\end{comment}

%% 150 words
\begin{comment}
Transport phenomena play a fundamental role in nuclear and plasma
physics, natural sciences, and engineering\textcolor{red}{. Yet,
}solving the associated high-dimensional advection-diffusion-reaction
equations remains a major computational challenge. We introduce the
Tensor Train Superconsistent Spectral (\mymethod{}) solver, a novel
approach that enables fast, accurate and stable
solutions \textcolor{red}{///////} in six-plus-time
dimensions. \mymethod{} \textcolor{red}{ combines} Spectral
Collocation for exponential convergence, Superconsistency
for \textcolor{red}{stabilization}, and the Tensor Train format for
extreme data compression. By enforcing a \textcolor{red}{suitable}
dimension-wise superconsistent condition compatible with tensor
structures, \mymethod{} achieves compression ratios of
$\mathcal{O}(10^{-12})$ while maintaining spectral
accuracy. \textcolor{red}{The} numerical experiments demonstrate
that \mymethod{} can solve six-plus-time dimensional transport
problems in minutes on standard computing
hardware\textcolor{red}{. The same tasks would require an exaggerated
amount of time} on current supercomputers using traditional
methods. \textcolor{red}{The new suggested perspective may make}
previously intractable high-dimensional problems in transport physics
and engineering \textcolor{red}{computationally accessible}.
\end{comment}

\begin{comment}
We present the Tensor Train Superconsistent Spectral (\mymethod{})
solver, a groundbreaking approach for solving high-dimensional partial
differential equations addressing fundamental challenges of
computational cost, stability, and accuracy. Our method uniquely
combines three powerful mathematical frameworks: Spectral Collocation
Method for exponential convergence, Superconsistency for unconditional
stability and Tensor Train format for efficient data compression. By
implementing a novel dimension-wise superconsistent condition
compatible with tensor structures, we achieve remarkable compression
ratios of $\mathcal{O}(10^{-12})$ while maintaining spectral
accuracy. Our numerical experiments demonstrate that (\mymethod{}) can
solve six-plus-time dimensional transport problems in minutes on
standard hardware that requires millions of years using traditional
methods. The solver remains stable across all parameter regimes,
including extremely small diffusion coefficients
($\varepsilon=10^{-6}$), while accurately capturing complex phenomena
such as boundary layers and high-frequency solutions. This
breakthrough enables practical solutions to previously intractable
problems in nuclear physics, plasma dynamics, and semiconductor
modeling, effectively democratizing access to high-dimensional
numerical solutions.
\end{comment}

\begin{comment}
We present the Tensor Train Superconsistent Spectral (\mymethod{})
Solver, a groundbreaking approach for solving high-dimensional partial
differential equations that addresses the fundamental challenges of
computational cost, stability, and accuracy.
%%
Our method uniquely combines three powerful mathematical frameworks:
the Spectral Collocation Method for exponential convergence,
Superconsistency for unconditional stability, and the Tensor Train
format for efficient data compression.
%%
By implementing a novel dimension-wise superconsistent condition
compatible with tensor structures, we achieve remarkable compression
ratios of $\mathcal{O}(10^{-12})$ while maintaining spectral accuracy.
%%
Our numerical experiments demonstrate that (\mymethod{}) can solve
six-plus-time dimensional transport problems in minutes on standard
computing hardware—tasks that would require millions of years on
current supercomputers using traditional methods.
%%
The solver remains stable across all parameter regimes, including
extremely small diffusion coefficients ($\varepsilon=10^{-6}$), while
accurately capturing complex phenomena such as boundary layers and
high-frequency solutions.
%%
This breakthrough enables the practical solution of previously
intractable problems in nuclear physics, plasma dynamics, and
semiconductor modeling, effectively democratizing access to
high-dimensional numerical solutions.
\end{comment}

Transport phenomena are the backbone of nuclear and plasma physics,
natural sciences and engineering.
%%
However, solving the associated high-dimensional
convection-diffusion-reaction equations remains a major computational
challenge.
%%
We introduce the Tensor Train Superconsistent Spectral (\mymethod{})
solver, a numerical approach that, through the combination of
different solution techniques, enables fast, accurate, and
oscillation-free solutions of multidimensional transport equations.
%%
We focus, in particular, on the in six plus time dimensional case for
its relevance in plasma physics numerical simualtion, e.g.,
Vlasov-like models.
%%
\mymethod{} leverages spectral collocation for exponential convergence,
superconsistency for stabilization in the transport-dominated regime,
and the tensor train format for extreme data compression.
%%
By enforcing a suitable dimension-wise superconsistent condition
compatible with tensor structures, \mymethod{} achieves compression
ratios of $\mathcal{O}(10^{-12})$ while preserving spectral accuracy.
%%
Numerical experiments conducted on some linear problems demonstrate
that
\mymethod{} can solve high-dimensional transport problems in minutes on
standard computing hardware, making previously intractable problems in
transport physics and engineering computationally accessible.  (132
words)


==> agenda_sunt.tex <==
\section*{Agenda Sunt}

\begin{itemize}
\item $\times$\textbf{Daniele}: please, guarda le ultime correzioni
  che ho fatto (in magenta) se ti vanno bene
\item $\times$\textbf{Nicola:} please, aggiungi l'info che manca a
  pagina 8 (le pagine si riferiscono alla mai versione)
\item $\times$\textbf{Nicola:} please, controlla la Section 5.3
  (l'ultima) che il modo in cui ho descritto l codice sia corretto
\item $\times$\textbf{Nicola:} dove controlliamo i ranghi con il
  rounding? Lo fa AMEn? Qual'e` la tolerance?
\item $\times$\textbf{TUTTI}: cosa facciamo con il test a pagina 7-8
  (vedi magenta)? Lo teniamo, lo togliamo, oppure facciamo un altro
  test? \`E giusto il commento che ho scritto, cio\`e che lo schema
  non usa la superconsistenza perch\'e si accorge che non ce ne \`e
  bisogno?
\end{itemize}

%% \textcolor{blue}{Ho finito di dare una spolverata generale. Attendo
%% le vostre correzioni. Daniele}

%% \MGT{[Marco]: Nicola (e Andrea), please, fate una passata eliminando tutto il "rosso" possibile di Daniele. Appena avete fatto, lo prendo in mano io per una riguardata finale. Per andare pi\`u veloci, in parallelo nei prossimi giorni lavoro sulla parte Methods, che mi compete direttamente. Le Conclusions (sorry, vengo da una scuola "diversa" in merito ai papers, e di solito scrivo sempre una section con le Conclusions alla fine), si possono eliminare dal fondo e se c'\`e qualche osservazione utile o significativa, si pu\`o fare il merge con la Discussion. Abbiamo gi\`a un LA-UR per cui appena finiamo si potrebbe sottomettere. Tuttavia, siccome questa versione sta venendo un p\`o diversa da quella che ho sottomesso, vorrei fare un update del LA-UR con la versione finale prima di mandarlo alla rivista (non sarebbe strettamente richiesto, ma \`e bene farlo).}
%% \textcolor{cyan}{{C}oncordo. Per Methods: la figura che ha preparato Nicola sui TT e' utile da aggiungere all'inizio della section sui TT. In questi articoli la section Discussion e' molto importante. Nella revisione dobbiamo anche essere capaci di bilanciare un "low profile" (saranno i lettori a dire il valore) ma chiarezza del valore quantitativo dei risultati del metodo. E con una prospettiva differente qual sarebbe il vantaggio del metodo su un supercomputer...}
%% \begin{enumerate}
%%     \item Correct Reynolds 
%%     \item Teniamo 7 domensionale oppure $6+$tempo?

%%     \item \sout{“Advection dominant” è un attributo del prototipo, non del modello (analitico o numerico). 
%%     Fa riferimento agli alti numeri di Reynolds o Peclet, rispettivamente rapporto 
%%     di velocità o trasporto di massa versus viscosità, 
%%     \href{https://en.wikipedia.org/wiki/Moody_chart}{questo grafico}, un diagramma molto importante nei corsi di meccanica dei fluidi, 
%%     mostra bene che un solutore Advection Dominant deve essere robusto rispetto a 
%%     Reynolds fino a $10^7$ / $10^8$. 
%%     Sia Re che Pe sono fratelli gemelli (invertiti, scostumati) 
%%     del nostro $\varepsilon / \beta L$, 
%%     in questo modo i nostri “clienti” possono immediatamente capire che 
%%     T2S2 e’ utile alle loro applicazioni. Credo che nel paper 
%%     lo abbiamo scritto sbagliato al momento, \textsc{Agenda}: dobbiamo correggerlo.} 
    
%%     \item \sout{Il ruolo di $n$.  Per quanto TT ci consenta di 
%%     arrivare ad $n_i$ molto grandi, non arriviamo mai ad infinito, 
%%     o almeno un numero tale per cui i punti upwind tornino ad essere gli 
%%     zeri di $P'_n$}
    
%%     \item \sout{Il solutore lineare in formato tensor train si basa su un solutore diretto di 
%%     complessità $(r_{i-1} n_i r_i)^3$, con tutto il consumo di memoria dovuto al fatto 
%%     che le matrici del microlinearsystem sono, senza scampo, DENSE! 
%%     La figura 6 mostra come al limite delle capacità computazionali di 
%%     una workstation accettabile, grossa parte del regime di interesse del 
%%     rapporto $\varepsilon / \beta L$ sia ancora afflitto da 
%%     pesanti oscillazioni, mentre T2S2 no. \textsc{Agenda}: questo concetto c'era
%%     lo avamo tolto perche fondamentalmento non eroriuscito a spiegarlo bene. 
%%     Dobbiamo rimetterlo bene.}
    
%%     \item \sout{Riferimento ad El Capitan rimosso. 
%%     Si parla genericamente di exascale computing, specifichiamo che le ere geologiche 
%%     ci servono per dare un misura intuitiva di cosa significhi $10^{18}$ secondi. }
    
%%     \item \sout{In Figura 5 facciamo vedere che \emph(i) l’upwinding mantiene 
%%     la convergenza spettrale e che \emph(ii) il nostro solver per una soluzione di 
%%     rango basso mantiene rango basso. 
%%     Entrambi i risultati non erano scontati all'inizio della nostra esplorazione. 
%%     Questa referenza \cite{Einkemmer:2024} 
%%     spiega bene che e’ importante fare questa verifica su griglie 
%%     inaccessibili a solutori tradizionali. \textsc{Agenda}: rileggere overview 
%%     alla sezione risultati e controllare che questo sia specificato bene.}

%%     \item \sout{Figura 6: e’ l’estensione 6 dimensionale del test in figure 2.4.(1-2-3-4) 
%%     del libro di Daniele  ed e’ funzionale al punto 4.}
%% \end{enumerate}


==> defs.tex <==
%% Hey Emacs, this is -*-latex-*-

\usepackage{comment}
%% \usepackage[reqno]{amsmath}       %   AMS equation environments
\usepackage{amsmath}
\usepackage{amssymb}       %   AMS symbol fonts (e.g., \boldsymbol{}
\usepackage{amsthm}      %   conflicts with elsart style

\usepackage{chapterbib}    %   Bibtex
\usepackage{color}
\usepackage{comment}
\usepackage{bm,bbm}
\usepackage{overpic}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx,graphics,rotating}
\usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{siunitx}
\usepackage{booktabs}
\usepackage{soul}

% \usepackage[inkscape={/usr/bin/inkscape -z -C}]{svg}
% pdflatex --shell-escape main.tex

%\usepackage{hyperref}
%\usepackage[right,inline]{showlabels}
%\usepackage{mathtools}
%%\usepackage{listings}
%\usepackage{minted}
%\usemintedstyle{igor}

\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}

\theoremstyle{plain}
\newtheorem{assumption}[theorem]{Assumption}

%%%%%%%%%%%%%%% colors (you can change the colors if you do not like)
\definecolor{MyDarkGreen}{rgb}{0,0.45,0}
\newcommand{\Jerome}[1]{\noindent{\color{red}\textbf{[F:~#1]}}}
%\newcommand{\Marco} [1]{\noindent{\color{MyDarkGreen}\textbf{[Marco:~#1]}}}
%\newcommand{\Max}[1]{\noindent{\color{blue}[Max:~#1]}}
\newcommand{\Max}[1]{\noindent{\color{blue}#1}}
%%\newcommand{\Max}[1]{#1}

\newcommand{\BLK}[1]{\textcolor{black}{#1}}
\newcommand{\RED}[1]{\textcolor{red}{#1}}
\newcommand{\MGT}[1]{\textcolor{magenta}{#1}}               
\newcommand{\BLUE}[1]{\textcolor{blue}{#1}}

%% le petit carr{\'e} de fin de d{\'e}monstration
\def\trait #1 #2 #3 {\vrule width #1pt height #2pt depth #3pt}
\def\fin{\hfill
        \trait .3 5 0
        \trait 5 .3 0
        \kern-5pt
        \trait 5 5 -4.7
        \trait 0.3 5 0
\medskip}
\newcommand{\ENDPROOF}{\fin}

\setlength{\topmargin}{-0.25in}
\setlength{\textheight}{8.9in}%{20.5cm}
\setlength{\oddsidemargin}{-0.05in}
\setlength{\evensidemargin}{0.0in}

\setlength{\textwidth}{6.6in}%{15cm}

% \newenvironment{proof}{\textit{Proof. }}{\fin}

%% ------------------------------------------------------------------------------------------
%% 
%% WriteUps special commands
%% 
%% ------------------------------------------------------------------------------------------

\newif\ifANKI

\newcounter{numbs}
\newcounter{numbi}
\newcounter{numbii}

\ANKIfalse
%%\ANKItrue

\ifANKI

\newcommand{\NewItem}[1]{
  \stepcounter{numbi}
  \setcounter{numbii}{0}
  \clearpage
  \bigskip\noindent
  \textbf{\thenumbs.\thenumbi.}
  \medskip
  \noindent
  \PGRAPH{#1}~\\
  \clearpage
}

%% \renewcommand{\section}[1]{}

\else

\setcounter{numbs}{1}

\newcommand{\NewItem}[1]{
  \stepcounter{numbi}
  \setcounter{numbii}{0}
  \bigskip\noindent
  \textbf{\thenumbs.\thenumbi.}
  \medskip
  \noindent
  \PGRAPH{#1} %~\\
}

\fi

\newcommand{\SubItem}[1]{
  \stepcounter{numbii}
  \medskip\noindent
  \textbf{\thenumbs.\thenumbi.\thenumbii.}
  \PGRAPH{#1}
}

\newcommand{\SecItem}[1]
{
  \setcounter{numbi} {0}
  \stepcounter{numbs}
  \bigskip\medskip\noindent
  %\begin{large}
  \textbf{\!\!\thenumbs.~~#1}
  %\end{large}
}

\newcommand{\NewItemR}{\RED{\NewItem}}
\newcommand{\SubItemR}{\RED{\SubItem}}

\newcommand{\PGRAPH}[1]{\noindent\textbf{#1}}
%\newcommand{\PGRAPH}[1]{\medskip\noindent\textbf{#1}}
%\newcommand{\PSEC}[1]{\bigskip\bigskip\noindent\begin{large}\textbf{#1}\end{large}}

%% ------------------------------------------------------------------------------------------
%% 
%% ACRONYMS
%% 
%% ------------------------------------------------------------------------------------------

\newcommand{\MFD}{\text{MFD}}
\newcommand{\VEM}{\text{VEM}}
\newcommand{\FEM}{\text{FEM}}
\newcommand{\FVM}{\text{FVM}}
\newcommand{\HMM}{\text{HMM}}
\newcommand{\PPUM}{\text{P-PUM}}
\newcommand{\PUM}{\text{PUM}}
\newcommand{\PUFE}{\text{PUFE}}
\newcommand{\GDM}{\text{GDM}}
\newcommand{\MATLAB}{\text{MATLAB}}

%% ------------------------------------------------------------------------------------------
%% 
%% AUXILIARY
%% 
%% ------------------------------------------------------------------------------------------

%% other symbols
\newcommand{\KER} {\,\textit{ker}}
\newcommand{\IMG} {\,\textit{img}}
\newcommand{\COLS}{\,\textit{cols}}
\newcommand{\ROWS}{\,\textit{rows}}
\newcommand{\dims}{\,\textit{dim}}
\newcommand{\INTP}{\footnotesize{\texttt{I}}}
\newcommand{\SPAN}[1]{\mbox{\textrm{span}}\big\{#1\big\}}
\newcommand{\REAL}{\mathbbm{R}}
\newcommand{\INTG}{\mathbbm{N}}
\newcommand{\CARD}[1]{\#{\left(#1\right)}}
\newcommand{\ASSUM}[1]{\textbf{(#1)}}
\newcommand{\HAT}[1]{\widehat{#1}}

\newcommand{\RANK}{\mbox{\textit{rank}}}

%% macros for text redaction
\newcommand{\TBW}{\textbf{To be written\ldots}}
\newcommand{\BIB}{[\textbf{BIB}]}
\newcommand{\CITE} [1]{[\textbf{Cite~#1}]}
\newcommand{\FNOTE}[1]{{\footnote{\textbf{#1}}}}
\newcommand{\ADDNOTE}[1]{\RED{\textbf{[#1]}}}
\newcommand{\ADDCITS}{\RED{\textbf{[Add Cits!]}}}
%% ------------------------------------------------------------------------------------------
%%
%% vectors
%%
%% ------------------------------------------------------------------------------------------

\newcommand{\av}{\mathbf{a}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\ccv}{\mathbf{c}}
\newcommand{\dv}{\mathbf{d}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\fv}{\mathbf{f}}
\newcommand{\gv}{\mathbf{g}}
\newcommand{\hv}{\mathbf{h}}
\newcommand{\iv}{\mathbf{i}}
\newcommand{\jv}{\mathbf{j}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\lv}{\mathbf{l}}
\newcommand{\mv}{\mathbf{m}}
\newcommand{\nv}{\mathbf{n}}
\newcommand{\ov}{\mathbf{o}}
\newcommand{\pv}{\mathbf{p}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\tv}{\mathbf{t}}
\newcommand{\uv}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\wv}{\mathbf{w}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\yv}{\mathbf{y}}
\newcommand{\zv}{\mathbf{z}}

\newcommand{\Av}{\mathbf{A}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\Cv}{\mathbf{C}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Ev}{\mathbf{E}}
\newcommand{\Fv}{\mathbf{F}}
\newcommand{\Gv}{\mathbf{G}}
\newcommand{\Hv}{\mathbf{H}}
\newcommand{\Iv}{\mathbf{I}}
\newcommand{\Jv}{\mathbf{J}}
\newcommand{\Kv}{\mathbf{K}}
\newcommand{\Lv}{\mathbf{L}}
\newcommand{\Mv}{\mathbf{M}}
\newcommand{\Nv}{\mathbf{N}}
\newcommand{\Ov}{\mathbf{O}}
\newcommand{\Pv}{\mathbf{P}}
\newcommand{\Qv}{\mathbf{Q}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\Sv}{\mathbf{S}}
\newcommand{\Tv}{\mathbf{T}}
\newcommand{\Uv}{\mathbf{U}}
\newcommand{\Vv}{\mathbf{V}}
\newcommand{\Wv}{\mathbf{W}}
\newcommand{\RX}{\mathbf{X}}
\newcommand{\RY}{\mathbf{Y}}
\newcommand{\Zv}{\mathbf{Z}}

\newcommand{\avv}[1]{\av_{#1}}
\newcommand{\bvv}[1]{\bv_{#1}}
\newcommand{\cvv}[1]{\cv_{#1}}
\newcommand{\dvv}[1]{\dv_{#1}}
\newcommand{\evv}[1]{\ev_{#1}}
\newcommand{\fvv}[1]{\fv_{#1}}
\newcommand{\gvv}[1]{\gv_{#1}}
\newcommand{\hvv}[1]{\hv_{#1}}
\newcommand{\ivv}[1]{\iv_{#1}}
\newcommand{\jvv}[1]{\jv_{#1}}
\newcommand{\kvv}[1]{\kv_{#1}}
\newcommand{\lvv}[1]{\lv_{#1}}
\newcommand{\mvv}[1]{\mv_{#1}}
\newcommand{\nvv}[1]{\nv_{#1}}
\newcommand{\ovv}[1]{\ov_{#1}}
\newcommand{\pvv}[1]{\pv_{#1}}
\newcommand{\qvv}[1]{\qv_{#1}}
\newcommand{\rvv}[1]{\rv_{#1}}
\newcommand{\svv}[1]{\sv_{#1}}
\newcommand{\tvv}[1]{\tv_{#1}}
\newcommand{\uvv}[1]{\uv_{#1}}
\newcommand{\vvv}[1]{\vv_{#1}}
\newcommand{\wvv}[1]{\wv_{#1}}
\newcommand{\xvv}[1]{\xv_{#1}}
\newcommand{\yvv}[1]{\yv_{#1}}
\newcommand{\zvv}[1]{\zv_{#1}}

\newcommand{\Avv}[1]{\Av_{#1}}
\newcommand{\Bvv}[1]{\Bv_{#1}}
\newcommand{\Cvv}[1]{\Cv_{#1}}
\newcommand{\Dvv}[1]{\Dv_{#1}}
\newcommand{\Evv}[1]{\Ev_{#1}}
\newcommand{\Fvv}[1]{\Fv_{#1}}
\newcommand{\Gvv}[1]{\Gv_{#1}}
\newcommand{\Hvv}[1]{\Hv_{#1}}
\newcommand{\Ivv}[1]{\Iv_{#1}}
\newcommand{\Jvv}[1]{\Jv_{#1}}
\newcommand{\Kvv}[1]{\Kv_{#1}}
\newcommand{\Lvv}[1]{\Lv_{#1}}
\newcommand{\Mvv}[1]{\Mv_{#1}}
\newcommand{\Nvv}[1]{\Nv_{#1}}
\newcommand{\Ovv}[1]{\Ov_{#1}}
\newcommand{\Pvv}[1]{\Pv_{#1}}
\newcommand{\Qvv}[1]{\Qv_{#1}}
\newcommand{\Rvv}[1]{\Rv_{#1}}
\newcommand{\Svv}[1]{\Sv_{#1}}
\newcommand{\Tvv}[1]{\Tv_{#1}}
\newcommand{\Uvv}[1]{\Uv_{#1}}
\newcommand{\Vvv}[1]{\Vv_{#1}}
\newcommand{\Wvv}[1]{\Wv_{#1}}
\newcommand{\Xvv}[1]{\Xv_{#1}}
\newcommand{\Yvv}[1]{\Yv_{#1}}
\newcommand{\Zvv}[1]{\Zv_{#1}}

\newcommand{\avs}[1]{\av^{#1}}
\newcommand{\bvs}[1]{\bv^{#1}}
\newcommand{\cvs}[1]{\cv^{#1}}
\newcommand{\dvs}[1]{\dv^{#1}}
\newcommand{\evs}[1]{\ev^{#1}}
\newcommand{\fvs}[1]{\fv^{#1}}
\newcommand{\gvs}[1]{\gv^{#1}}
\newcommand{\hvs}[1]{\hv^{#1}}
\newcommand{\ivs}[1]{\iv^{#1}}
\newcommand{\jvs}[1]{\jv^{#1}}
\newcommand{\kvs}[1]{\kv^{#1}}
\newcommand{\lvs}[1]{\lv^{#1}}
\newcommand{\mvs}[1]{\mv^{#1}}
\newcommand{\nvs}[1]{\nv^{#1}}
\newcommand{\ovs}[1]{\ov^{#1}}
\newcommand{\pvs}[1]{\pv^{#1}}
\newcommand{\qvs}[1]{\qv^{#1}}
\newcommand{\rvs}[1]{\rv^{#1}}
\newcommand{\svs}[1]{\sv^{#1}}
\newcommand{\tvs}[1]{\tv^{#1}}
\newcommand{\uvs}[1]{\uv^{#1}}
\newcommand{\vvs}[1]{\vv^{#1}}
\newcommand{\wvs}[1]{\wv^{#1}}
\newcommand{\xvs}[1]{\xv^{#1}}
\newcommand{\yvs}[1]{\yv^{#1}}
\newcommand{\zvs}[1]{\zv^{#1}}

\newcommand{\Avs}[1]{\Av^{#1}}
\newcommand{\Bvs}[1]{\Bv^{#1}}
\newcommand{\Cvs}[1]{\Cv^{#1}}
\newcommand{\Dvs}[1]{\Dv^{#1}}
\newcommand{\Evs}[1]{\Ev^{#1}}
\newcommand{\Fvs}[1]{\Fv^{#1}}
\newcommand{\Gvs}[1]{\Gv^{#1}}
\newcommand{\Hvs}[1]{\Hv^{#1}}
\newcommand{\Ivs}[1]{\Iv^{#1}}
\newcommand{\Jvs}[1]{\Jv^{#1}}
\newcommand{\Kvs}[1]{\Kv^{#1}}
\newcommand{\Lvs}[1]{\Lv^{#1}}
\newcommand{\Mvs}[1]{\Mv^{#1}}
\newcommand{\Nvs}[1]{\Nv^{#1}}
\newcommand{\Ovs}[1]{\Ov^{#1}}
\newcommand{\Pvs}[1]{\Pv^{#1}}
\newcommand{\Qvs}[1]{\Qv^{#1}}
\newcommand{\Rvs}[1]{\Rv^{#1}}
\newcommand{\Svs}[1]{\Sv^{#1}}
\newcommand{\Tvs}[1]{\Tv^{#1}}
\newcommand{\Uvs}[1]{\Uv^{#1}}
\newcommand{\Vvs}[1]{\Vv^{#1}}
\newcommand{\Wvs}[1]{\Wv^{#1}}
\newcommand{\Xvs}[1]{\Xv^{#1}}
\newcommand{\Yvs}[1]{\Yv^{#1}}
\newcommand{\Zvs}[1]{\Zv^{#1}}

%% vectors with a subindex and a superindex
\newcommand{\avz}[2]{\av_{#1}^{#2}}
\newcommand{\bvz}[2]{\bv_{#1}^{#2}}
\newcommand{\cvz}[2]{\cv_{#1}^{#2}}
\newcommand{\dvz}[2]{\dv_{#1}^{#2}}
\newcommand{\evz}[2]{\ev_{#1}^{#2}}
\newcommand{\fvz}[2]{\fv_{#1}^{#2}}
\newcommand{\gvz}[2]{\gv_{#1}^{#2}}
\newcommand{\hvz}[2]{\hv_{#1}^{#2}}
\newcommand{\ivz}[2]{\iv_{#1}^{#2}}
\newcommand{\jvz}[2]{\jv_{#1}^{#2}}
\newcommand{\kvz}[2]{\kv_{#1}^{#2}}
\newcommand{\lvz}[2]{\lv_{#1}^{#2}}
\newcommand{\mvz}[2]{\mv_{#1}^{#2}}
\newcommand{\nvz}[2]{\nv_{#1}^{#2}}
\newcommand{\ovz}[2]{\ov_{#1}^{#2}}
\newcommand{\pvz}[2]{\pv_{#1}^{#2}}
\newcommand{\qvz}[2]{\qv_{#1}^{#2}}
\newcommand{\rvz}[2]{\rv_{#1}^{#2}}
\newcommand{\szv}[2]{\sv_{#1}^{#2}}
\newcommand{\tvz}[2]{\tv_{#1}^{#2}}
\newcommand{\uvz}[2]{\uv_{#1}^{#2}}
\newcommand{\vvz}[2]{\vv_{#1}^{#2}}
\newcommand{\wvz}[2]{\wv_{#1}^{#2}}
\newcommand{\xvz}[2]{\xv_{#1}^{#2}}
\newcommand{\yvz}[2]{\yv_{#1}^{#2}}
\newcommand{\zvz}[2]{\zv_{#1}^{#2}}

\newcommand{\Avz}[2]{\Av_{#1}^{#2}}
\newcommand{\Bvz}[2]{\Bv_{#1}^{#2}}
\newcommand{\Cvz}[2]{\Cv_{#1}^{#2}}
\newcommand{\Dvz}[2]{\Dv_{#1}^{#2}}
\newcommand{\Evz}[2]{\Ev_{#1}^{#2}}
\newcommand{\Fvz}[2]{\Fv_{#1}^{#2}}
\newcommand{\Gvz}[2]{\Gv_{#1}^{#2}}
\newcommand{\Hvz}[2]{\Hv_{#1}^{#2}}
\newcommand{\Ivz}[2]{\Iv_{#1}^{#2}}
\newcommand{\Jvz}[2]{\Jv_{#1}^{#2}}
\newcommand{\Kvz}[2]{\Kv_{#1}^{#2}}
\newcommand{\Lvz}[2]{\Lv_{#1}^{#2}}
\newcommand{\Mvz}[2]{\Mv_{#1}^{#2}}
\newcommand{\Nvz}[2]{\Nv_{#1}^{#2}}
\newcommand{\Ovz}[2]{\Ov_{#1}^{#2}}
\newcommand{\Pvz}[2]{\Pv_{#1}^{#2}}
\newcommand{\Qvz}[2]{\Qv_{#1}^{#2}}
\newcommand{\Rvz}[2]{\Rv_{#1}^{#2}}
\newcommand{\Svz}[2]{\Sv_{#1}^{#2}}
\newcommand{\Tvz}[2]{\Tv_{#1}^{#2}}
\newcommand{\Uvz}[2]{\Uv_{#1}^{#2}}
\newcommand{\Vvz}[2]{\Vv_{#1}^{#2}}
\newcommand{\Wvz}[2]{\Wv_{#1}^{#2}}
\newcommand{\Xvz}[2]{\Xv_{#1}^{#2}}
\newcommand{\Yvz}[2]{\Yv_{#1}^{#2}}
\newcommand{\Zvz}[2]{\Zv_{#1}^{#2}}

%% ------------------------------------------------------------------------------------------
%%
%% scalars
%%
%% ------------------------------------------------------------------------------------------

\newcommand{\as}{a}
\newcommand{\bs}{b}
\newcommand{\cs}{c}
\newcommand{\ds}{d}
\newcommand{\es}{e}
\newcommand{\fs}{f}
\newcommand{\gs}{g}
\newcommand{\hs}{h}
\newcommand{\is}{i}
\newcommand{\js}{j}
\newcommand{\ks}{k}
\newcommand{\ls}{l}
\newcommand{\ms}{m}
\newcommand{\ns}{n}
\newcommand{\os}{o}
\newcommand{\ps}{p}
\newcommand{\qs}{q}
\newcommand{\rs}{r}
\renewcommand{\ss}{s}
\newcommand{\ts}{t}
\newcommand{\us}{u}
\newcommand{\vs}{v}
\newcommand{\ws}{w}
\newcommand{\xs}{x}
\newcommand{\ys}{y}
\newcommand{\zs}{z}

%% special cases
\newcommand{\usp}{\us^{\prime}}
\newcommand{\uspp}{\us^{\prime\prime}}

\newcommand{\As}{A}
\newcommand{\Bs}{B}
\newcommand{\Cs}{C}
\newcommand{\Ds}{D}
\newcommand{\Es}{E}
\newcommand{\Fs}{F}
\newcommand{\Gs}{G}
\newcommand{\Hs}{H}
\newcommand{\Is}{I}
\newcommand{\Js}{J}
\newcommand{\Ks}{K}
\newcommand{\Ls}{L}
\newcommand{\Ms}{M}
\newcommand{\Ns}{N}
\newcommand{\Os}{O}
\newcommand{\Ps}{P}
\newcommand{\Qs}{Q}
\newcommand{\Rs}{R}
\newcommand{\Ss}{S}
\newcommand{\Ts}{T}
\newcommand{\Us}{U}
\newcommand{\Vs}{V}
\newcommand{\Ws}{W}
\newcommand{\Xs}{X}
\newcommand{\Ys}{Y}
\newcommand{\Zs}{Z}

%% special cases
\newcommand{\Nsx}{\ns_x}
\newcommand{\Nsy}{\ns_y}
\newcommand{\Nsz}[2]{\Ns_{#1}^{#2}}
\newcommand{\Nst}{\ns_t}   

\newcommand{\asH}{\HAT{a}}
\newcommand{\bsH}{\HAT{b}}
\newcommand{\csH}{\HAT{c}}
\newcommand{\dsH}{\HAT{d}}
\newcommand{\esH}{\HAT{e}}
\newcommand{\fsH}{\HAT{f}}
\newcommand{\gsH}{\HAT{g}}
\newcommand{\hsH}{\HAT{h}}
\newcommand{\isH}{\HAT{i}}
\newcommand{\jsH}{\HAT{j}}
\newcommand{\ksH}{\HAT{k}}
\newcommand{\lsH}{\HAT{l}}
\newcommand{\msH}{\HAT{m}}
\newcommand{\nsH}{\HAT{n}}
\newcommand{\osH}{\HAT{o}}
\newcommand{\psH}{\HAT{p}}
\newcommand{\qsH}{\HAT{q}}
\newcommand{\rsH}{\HAT{r}}
\newcommand{\ssH}{\HAT{s}}
\newcommand{\tsH}{\HAT{t}}
\newcommand{\usH}{\HAT{u}}
\newcommand{\vsH}{\HAT{v}}
\newcommand{\wsH}{\HAT{w}}
\newcommand{\xsH}{\HAT{x}}
\newcommand{\ysH}{\HAT{y}}
\newcommand{\zsH}{\HAT{z}}

\newcommand{\AsH}{\HAT{A}}
\newcommand{\BsH}{\HAT{B}}
\newcommand{\CsH}{\HAT{C}}
\newcommand{\DsH}{\HAT{D}}
\newcommand{\EsH}{\HAT{E}}
\newcommand{\FsH}{\HAT{F}}
\newcommand{\GsH}{\HAT{G}}
\newcommand{\HsH}{\HAT{H}}
\newcommand{\IsH}{\HAT{I}}
\newcommand{\JsH}{\HAT{J}}
\newcommand{\KsH}{\HAT{K}}
\newcommand{\LsH}{\HAT{L}}
\newcommand{\MsH}{\HAT{M}}
\newcommand{\NsH}{\HAT{N}}
\newcommand{\OsH}{\HAT{O}}
\newcommand{\PsH}{\HAT{P}}
\newcommand{\QsH}{\HAT{Q}}
\newcommand{\RsH}{\HAT{R}}
\newcommand{\SsH}{\HAT{S}}
\newcommand{\TsH}{\HAT{T}}
\newcommand{\UsH}{\HAT{U}}
\newcommand{\VsH}{\HAT{V}}
\newcommand{\WsH}{\HAT{W}}
\newcommand{\XsH}{\HAT{X}}
\newcommand{\YsH}{\HAT{Y}}
\newcommand{\ZsH}{\HAT{Z}}

\newcommand{\asb}{\overline{a}}
\newcommand{\bsb}{\overline{b}}
\newcommand{\csb}{\overline{c}}
\newcommand{\dsb}{\overline{d}}
\newcommand{\esb}{\overline{e}}
\newcommand{\fsb}{\overline{f}}
\newcommand{\gsb}{\overline{g}}
\newcommand{\hsb}{\overline{h}}
\newcommand{\isb}{\overline{i}}
\newcommand{\jsb}{\overline{j}}
\newcommand{\ksb}{\overline{k}}
\newcommand{\lsb}{\overline{l}}
\newcommand{\msb}{\overline{m}}
\newcommand{\nsb}{\overline{n}}
\newcommand{\osb}{\overline{o}}
\newcommand{\psb}{\overline{p}}
\newcommand{\qsb}{\overline{q}}
\newcommand{\rsb}{\overline{r}}
\newcommand{\ssb}{\overline{s}}
\newcommand{\tsb}{\overline{t}}
\newcommand{\usb}{\overline{u}}
\newcommand{\vsb}{\overline{v}}
\newcommand{\wsb}{\overline{w}}
\newcommand{\xsb}{\overline{x}}
\newcommand{\ysb}{\overline{y}}
\newcommand{\zsb}{\overline{z}}

\newcommand{\Asb}{\overline{A}}
\newcommand{\Bsb}{\overline{B}}
\newcommand{\Csb}{\overline{C}}
\newcommand{\Dsb}{\overline{D}}
\newcommand{\Esb}{\overline{E}}
\newcommand{\Fsb}{\overline{F}}
\newcommand{\Gsb}{\overline{G}}
\newcommand{\Hsb}{\overline{H}}
\newcommand{\Isb}{\overline{I}}
\newcommand{\Jsb}{\overline{J}}
\newcommand{\Ksb}{\overline{K}}
\newcommand{\Lsb}{\overline{L}}
\newcommand{\Msb}{\overline{M}}
\newcommand{\Nsb}{\overline{N}}
\newcommand{\Osb}{\overline{O}}
\newcommand{\Psb}{\overline{P}}
\newcommand{\Qsb}{\overline{Q}}
\newcommand{\Rsb}{\overline{R}}
\newcommand{\Ssb}{\overline{S}}
\newcommand{\Tsb}{\overline{T}}
\newcommand{\Usb}{\overline{U}}
\newcommand{\Vsb}{\overline{V}}
\newcommand{\Wsb}{\overline{W}}
\newcommand{\Xsb}{\overline{X}}
\newcommand{\Ysb}{\overline{Y}}
\newcommand{\Zsb}{\overline{Z}}

\newcommand{\asu}{\underline{a}}
\newcommand{\bsu}{\underline{b}}
\newcommand{\csu}{\underline{c}}
\newcommand{\dsu}{\underline{d}}
\newcommand{\esu}{\underline{e}}
\newcommand{\fsu}{\underline{f}}
\newcommand{\gsu}{\underline{g}}
\newcommand{\hsu}{\underline{h}}
\newcommand{\isu}{\underline{i}}
\newcommand{\jsu}{\underline{j}}
\newcommand{\ksu}{\underline{k}}
\newcommand{\lsu}{\underline{l}}
\newcommand{\msu}{\underline{m}}
\newcommand{\nsu}{\underline{n}}
\newcommand{\osu}{\underline{o}}
\newcommand{\psu}{\underline{p}}
\newcommand{\qsu}{\underline{q}}
\newcommand{\rsu}{\underline{r}}
\newcommand{\ssu}{\underline{s}}
\newcommand{\tsu}{\underline{t}}
\newcommand{\usu}{\underline{u}}
\newcommand{\vsu}{\underline{v}}
\newcommand{\wsu}{\underline{w}}
\newcommand{\xsu}{\underline{x}}
\newcommand{\ysu}{\underline{y}}
\newcommand{\zsu}{\underline{z}}

\renewcommand{\ast}{\widetilde{a}}
\newcommand{\bst}{\widetilde{b}}
\newcommand{\cst}{\widetilde{c}}
\newcommand{\dst}{\widetilde{d}}
\newcommand{\est}{\widetilde{e}}
\newcommand{\fst}{\widetilde{f}}
\newcommand{\gst}{\widetilde{g}}
\newcommand{\hst}{\widetilde{h}}
\newcommand{\ist}{\widetilde{i}}
\newcommand{\jst}{\widetilde{j}}
\newcommand{\kst}{\widetilde{k}}
\newcommand{\lst}{\widetilde{l}}
\newcommand{\mst}{\widetilde{m}}
\newcommand{\nst}{\widetilde{n}}
\newcommand{\ost}{\widetilde{o}}
\newcommand{\pst}{\widetilde{p}}
\newcommand{\qst}{\widetilde{q}}
\newcommand{\rst}{\widetilde{r}}
\newcommand{\sst}{\widetilde{s}}
\newcommand{\tst}{\widetilde{t}}
\newcommand{\ust}{\widetilde{u}}
\newcommand{\vst}{\widetilde{v}}
\newcommand{\wst}{\widetilde{w}}
\newcommand{\xst}{\widetilde{x}}
\newcommand{\yst}{\widetilde{y}}
\newcommand{\zst}{\widetilde{z}}

\newcommand{\Ast}{\widetilde{A}}
\newcommand{\Bst}{\widetilde{B}}
\newcommand{\Cst}{\widetilde{C}}
\newcommand{\Dst}{\widetilde{D}}
\newcommand{\Est}{\widetilde{E}}
\newcommand{\Fst}{\widetilde{F}}
\newcommand{\Gst}{\widetilde{G}}
\newcommand{\Hst}{\widetilde{t}}
\newcommand{\Ist}{\widetilde{I}}
\newcommand{\Jst}{\widetilde{J}}
\newcommand{\Kst}{\widetilde{K}}
\newcommand{\Lst}{\widetilde{L}}
\newcommand{\Mst}{\widetilde{M}}
\newcommand{\Nstt}{\widetilde{N}}
\newcommand{\Ost}{\widetilde{O}}
\newcommand{\Pst}{\widetilde{P}}
\newcommand{\Qst}{\widetilde{Q}}
\newcommand{\Rst}{\widetilde{R}}
\newcommand{\Sst}{\widetilde{S}}
\newcommand{\Tst}{\widetilde{T}}
\newcommand{\Ust}{\widetilde{U}}
\newcommand{\Vst}{\widetilde{V}}
\newcommand{\Wst}{\widetilde{W}}
\newcommand{\Xst}{\widetilde{X}}
\newcommand{\Yst}{\widetilde{Y}}
\newcommand{\Zst}{\widetilde{Z}}

%% ------------------------------------------------------------------------------------------
%%
%% scalars with subindex
%%
%% ------------------------------------------------------------------------------------------

\newcommand{\ass}[1]{a_{#1}}
\newcommand{\bss}[1]{b_{#1}}
\newcommand{\css}[1]{c_{#1}}
\newcommand{\dss}[1]{d_{#1}}
\newcommand{\ess}[1]{e_{#1}}
\newcommand{\fss}[1]{f_{#1}}
\newcommand{\gss}[1]{g_{#1}}
%%\renewcommand{\hss}[1]{h_{#1}}
\newcommand{\iss}[1]{i_{#1}}
\newcommand{\jss}[1]{j_{#1}}
\newcommand{\kss}[1]{k_{#1}}
\newcommand{\lss}[1]{l_{#1}}
\newcommand{\mss}[1]{m_{#1}}
\newcommand{\nss}[1]{n_{#1}}
\newcommand{\oss}[1]{o_{#1}}
\newcommand{\pss}[1]{p_{#1}}
\newcommand{\qss}[1]{q_{#1}}
\newcommand{\rss}[1]{r_{#1}}
\newcommand{\sss}[1]{s_{#1}}
\newcommand{\tss}[1]{t_{#1}}
\newcommand{\uss}[1]{u_{#1}}
%% \renewcommand{\vss}[1]{v_{#1}} %% conflicts with overpic !!!!
\newcommand{\wss}[1]{w_{#1}}
\newcommand{\xss}[1]{x_{#1}}
\newcommand{\yss}[1]{y_{#1}}
\newcommand{\zss}[1]{z_{#1}}

\newcommand{\Ass}[1]{A_{#1}}
\newcommand{\Bss}[1]{B_{#1}}
\newcommand{\Css}[1]{C_{#1}}
\newcommand{\Dss}[1]{D_{#1}}
\newcommand{\Ess}[1]{E_{#1}}
\newcommand{\Fss}[1]{F_{#1}}
\newcommand{\Gss}[1]{G_{#1}}
\newcommand{\Hss}[1]{H_{#1}}
\newcommand{\Iss}[1]{I_{#1}}
\newcommand{\Jss}[1]{J_{#1}}
\newcommand{\Kss}[1]{K_{#1}}
\newcommand{\Lss}[1]{L_{#1}}
\newcommand{\Mss}[1]{M_{#1}}
\newcommand{\Nss}[1]{N_{#1}}
\newcommand{\Oss}[1]{O_{#1}}
\newcommand{\Pss}[1]{P_{#1}}
\newcommand{\Qss}[1]{Q_{#1}}
\newcommand{\Rss}[1]{R_{#1}}
\newcommand{\Sss}[1]{S_{#1}}
\newcommand{\Tss}[1]{T_{#1}}
\newcommand{\Uss}[1]{U_{#1}}
\newcommand{\Vss}[1]{V_{#1}}
\newcommand{\Wss}[1]{W_{#1}}
\newcommand{\Xss}[1]{X_{#1}}
\newcommand{\Yss}[1]{Y_{#1}}
\newcommand{\Zss}[1]{Z_{#1}}

%% vectors with a subindex and a superindex
\newcommand{\asz}[2]{\as_{#1}^{#2}}
\newcommand{\bsz}[2]{\bs_{#1}^{#2}}
\newcommand{\csz}[2]{\cs_{#1}^{#2}}
\newcommand{\dsz}[2]{\ds_{#1}^{#2}}
\newcommand{\esz}[2]{\es_{#1}^{#2}}
\newcommand{\fsz}[2]{\fs_{#1}^{#2}}
\newcommand{\gsz}[2]{\gs_{#1}^{#2}}
\newcommand{\hsz}[2]{\hs_{#1}^{#2}}
\newcommand{\isz}[2]{\is_{#1}^{#2}}
\newcommand{\jsz}[2]{\js_{#1}^{#2}}
\newcommand{\ksz}[2]{\ks_{#1}^{#2}}
\newcommand{\lsz}[2]{\ls_{#1}^{#2}}
\newcommand{\msz}[2]{\ms_{#1}^{#2}}
\newcommand{\nsz}[2]{\ns_{#1}^{#2}}
\newcommand{\osz}[2]{\os_{#1}^{#2}}
\newcommand{\psz}[2]{\ps_{#1}^{#2}}
\newcommand{\qsz}[2]{\qs_{#1}^{#2}}
\newcommand{\rsz}[2]{\rs_{#1}^{#2}}
\newcommand{\ssz}[2]{\ss_{#1}^{#2}}
\newcommand{\tsz}[2]{\ts_{#1}^{#2}}
\newcommand{\usz}[2]{\us_{#1}^{#2}}
\newcommand{\vsz}[2]{\vs_{#1}^{#2}}
\newcommand{\wsz}[2]{\ws_{#1}^{#2}}
\newcommand{\xsz}[2]{\xs_{#1}^{#2}}
\newcommand{\ysz}[2]{\ys_{#1}^{#2}}
\newcommand{\zsz}[2]{\zs_{#1}^{#2}}

\newcommand{\Asz}[2]{\As_{#1}^{#2}}
\newcommand{\Bsz}[2]{\Bs_{#1}^{#2}}
\newcommand{\Csz}[2]{\Cs_{#1}^{#2}}
\newcommand{\Dsz}[2]{\Ds_{#1}^{#2}}
\newcommand{\Esz}[2]{\Es_{#1}^{#2}}
\newcommand{\Fsz}[2]{\Fs_{#1}^{#2}}
\newcommand{\Gsz}[2]{\Gs_{#1}^{#2}}
\newcommand{\Hsz}[2]{\Hs_{#1}^{#2}}
\newcommand{\Isz}[2]{\Is_{#1}^{#2}}
\newcommand{\Jsz}[2]{\Js_{#1}^{#2}}
\newcommand{\Ksz}[2]{\Ks_{#1}^{#2}}
\newcommand{\Lsz}[2]{\Ls_{#1}^{#2}}
\newcommand{\Msz}[2]{\Ms_{#1}^{#2}}
\newcommand{\Nszz}[2]{\Ns_{#1}^{#2}}
\newcommand{\Osz}[2]{\Os_{#1}^{#2}}
\newcommand{\Psz}[2]{\Ps_{#1}^{#2}}
\newcommand{\Qsz}[2]{\Qs_{#1}^{#2}}
\newcommand{\Rsz}[2]{\Rs_{#1}^{#2}}
\newcommand{\Ssz}[2]{\Ss_{#1}^{#2}}
\newcommand{\Tsz}[2]{\Ts_{#1}^{#2}}
\newcommand{\Usz}[2]{\Us_{#1}^{#2}}
\newcommand{\Vsz}[2]{\Vs_{#1}^{#2}}
\newcommand{\Wsz}[2]{\Ws_{#1}^{#2}}
\newcommand{\Xsz}[2]{\Xs_{#1}^{#2}}
\newcommand{\Ysz}[2]{\Ys_{#1}^{#2}}
\newcommand{\Zsz}[2]{\Zs_{#1}^{#2}}

%% ------------------------------------------------------------------------------------------
%%
%% matrices, pseudoinverse
%%
%% ------------------------------------------------------------------------------------------

\newcommand{\matA}{\mathsf{A}}
\newcommand{\matB}{\mathsf{B}}
\newcommand{\matC}{\mathsf{C}}
\newcommand{\matD}{\mathsf{D}}
\newcommand{\matE}{\mathsf{E}}
\newcommand{\matF}{\mathsf{F}}
\newcommand{\matG}{\mathsf{G}}
\newcommand{\matH}{\mathsf{H}}
\newcommand{\matI}{\mathsf{I}}
\newcommand{\matJ}{\mathsf{J}}
\newcommand{\matK}{\mathsf{K}}
\newcommand{\matL}{\mathsf{L}}
\newcommand{\matM}{\mathsf{M}}
\newcommand{\matN}{\mathsf{N}}
\newcommand{\matO}{\mathsf{O}}
\newcommand{\matP}{\mathsf{P}}
\newcommand{\matQ}{\mathsf{Q}}
\newcommand{\matR}{\mathsf{R}}
\newcommand{\matS}{\mathsf{S}}
\newcommand{\matT}{\mathsf{T}}
\newcommand{\matU}{\mathsf{U}}
\newcommand{\matV}{\mathsf{V}}
\newcommand{\matW}{\mathsf{W}}
\newcommand{\matX}{\mathsf{X}}
\newcommand{\matY}{\mathsf{Y}}
\newcommand{\matZ}{\mathsf{Z}}

\newcommand{\invA}{\matA^{\dagger}}
\newcommand{\invB}{\matB^{\dagger}}
\newcommand{\invC}{\matC^{\dagger}}
\newcommand{\invD}{\matD^{\dagger}}
\newcommand{\invE}{\matE^{\dagger}}
\newcommand{\invF}{\matF^{\dagger}}
\newcommand{\invG}{\matG^{\dagger}}
\newcommand{\invH}{\matH^{\dagger}}
\newcommand{\invI}{\matI^{\dagger}}
\newcommand{\invJ}{\matJ^{\dagger}}
\newcommand{\invK}{\matK^{\dagger}}
\newcommand{\invL}{\matL^{\dagger}}
\newcommand{\invM}{\matM^{\dagger}}
\newcommand{\invN}{\matN^{\dagger}}
\newcommand{\invO}{\matO^{\dagger}}
\newcommand{\invP}{\matP^{\dagger}}
\newcommand{\invQ}{\matQ^{\dagger}}
\newcommand{\invR}{\matR^{\dagger}}
\newcommand{\invS}{\matS^{\dagger}}
\newcommand{\invT}{\matT^{\dagger}}
\newcommand{\invU}{\matU^{\dagger}}
\newcommand{\invV}{\matV^{\dagger}}
\newcommand{\invW}{\matW^{\dagger}}
\newcommand{\invX}{\matX^{\dagger}}
\newcommand{\invY}{\matY^{\dagger}}
\newcommand{\invZ}{\matZ^{\dagger}}

\newcommand{\MATRIXFONT}[1]{\mathrm{#1}}
\newcommand{\mA}{\MATRIXFONT{A}}
\newcommand{\mB}{\MATRIXFONT{B}}
\newcommand{\mC}{\MATRIXFONT{C}}
\newcommand{\mD}{\MATRIXFONT{D}}
\newcommand{\mE}{\MATRIXFONT{E}}
\newcommand{\mF}{\MATRIXFONT{F}}
\newcommand{\mG}{\MATRIXFONT{G}}
\newcommand{\mH}{\MATRIXFONT{H}}
\newcommand{\mI}{\MATRIXFONT{I}}
\newcommand{\mJ}{\MATRIXFONT{J}}
\newcommand{\mK}{\MATRIXFONT{K}}
\newcommand{\mL}{\MATRIXFONT{L}}
\newcommand{\mM}{\MATRIXFONT{M}}
\newcommand{\mN}{\MATRIXFONT{N}}
\newcommand{\mO}{\MATRIXFONT{O}}
\newcommand{\mP}{\MATRIXFONT{P}}
\newcommand{\mQ}{\MATRIXFONT{Q}}
\newcommand{\mR}{\MATRIXFONT{R}}
\newcommand{\mS}{\MATRIXFONT{S}}
\newcommand{\mT}{\MATRIXFONT{T}}
\newcommand{\mU}{\MATRIXFONT{U}}
\newcommand{\mV}{\MATRIXFONT{V}}
\newcommand{\mW}{\MATRIXFONT{W}}
\newcommand{\mX}{\MATRIXFONT{X}}
\newcommand{\mY}{\MATRIXFONT{Y}}
\newcommand{\mZ}{\MATRIXFONT{Z}}

%% special
\newcommand{\invinvS}{\matS^{\dagger\dagger}}
\newcommand{\matAb}{\overline{\matA}}
\newcommand{\mAb}{\overline{\mA}}
\newcommand{\mat}{\textrm{mat}}

%% ------------------------------------------------------------------------------------------
%%
%% calligraphic symbols
%%
%% ------------------------------------------------------------------------------------------

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\tA}{\mathcal{A}}
\newcommand{\tB}{\mathcal{B}}
\newcommand{\tC}{\mathcal{C}}
\newcommand{\tD}{\mathcal{D}}
\newcommand{\tE}{\mathcal{E}}
\newcommand{\tF}{\mathcal{F}}
\newcommand{\tG}{\mathcal{G}}
\newcommand{\tH}{\mathcal{H}}
\newcommand{\tI}{\mathcal{I}}
\newcommand{\tJ}{\mathcal{J}}
\newcommand{\tK}{\mathcal{K}}
\newcommand{\tL}{\mathcal{L}}
\newcommand{\tM}{\mathcal{M}}
\newcommand{\tN}{\mathcal{N}}
\newcommand{\tO}{\mathcal{O}}
\newcommand{\tP}{\mathcal{P}}
\newcommand{\tQ}{\mathcal{Q}}
\newcommand{\tR}{\mathcal{R}}
\newcommand{\tS}{\mathcal{S}}
\newcommand{\tT}{\mathcal{T}}
\newcommand{\tU}{\mathcal{U}}
\newcommand{\tV}{\mathcal{V}}
\newcommand{\tW}{\mathcal{W}}
\newcommand{\tX}{\mathcal{X}}
\newcommand{\tY}{\mathcal{Y}}
\newcommand{\tZ}{\mathcal{Z}}

%% special commands
\newcommand{\calXht}{\widetilde{\calX}_{\hh}}
\newcommand{\calXh}{\calX_{\hh}}
\newcommand{\calEs}{\calE^*}
\newcommand{\tATT}{\mathcal{A}^{TT}}

%% ------------------------------------------------------------------------------------------
%% 
%% CONTINUOUS SETTING
%% 
%% ------------------------------------------------------------------------------------------

% domain
\newcommand{\GamD}{\Gamma_{\!D}}
\newcommand{\GamN}{\Gamma_{\!N}}

% functional spaces
\newcommand{\WSz}[1]{W^{#1}_0}
\newcommand{\PS}[1]{\mathbbm{P}_{#1}}
\newcommand{\PSz}[1]{\mathbbm{P}_{#1}^0}
\newcommand{\PSt}[1]{\widetilde{\mathbbm{P}}_{#1}}
\newcommand{\PShat}[1]{\mathbbm{\widehat{P}}_{#1}}

\newcommand{\HONE}   {H^1}
\newcommand{\HONEzr} {H^1_0}
\newcommand{\HONEnc} {H^{1,nc}_{\periodic}}
\newcommand{\HONEnck}{H^{1,nc}_{k}}
\newcommand{\HTWO}   {H^2}

\newcommand{\LP}    {L^p}
\newcommand{\LONE}  {L^1}
\newcommand{\LTWO}  {L^2}
\newcommand{\LINF}  {L^{\infty}}

\newcommand{\WS}[2] {W^{#1}_{#2}}
\newcommand{\LS}[1] {L^{#1}}
\newcommand{\HS}[1] {H^{#1}}
\newcommand{\BS}[1] {B_{#1}}
\newcommand{\QS}[1] {\mathbbm{Q}_{#1}}
\newcommand{\QSPU}[1] {\mathbbm{Q}^{\textrm{PU}}_{#1}}
\newcommand{\QSPUu}[1]{\underline{\mathbbm{Q}}^{\textrm{PU}}_{#1}}
\newcommand{\CS}[1] {C^{#1}}

\newcommand{\VS}[1] {V^{#1}}
\newcommand{\VSu}[1]{\underline{V}^{#1}}
\newcommand{\Vspace}{\VS{}}

\newcommand{\HDIV}{H(\textrm{div};\Omega)}
\newcommand{\HDIVpr}{\HONE_{\periodic}(\textrm{div};\Omega)}

\newcommand{\periodic}{p}
\newcommand{\HONEpr}{H^1_{\periodic}}
%% \newcommand{\LTWOpr}{L^2_{\periodic}}
%% \newcommand{\HSpr}[1]{H^{#1}_{\periodic}}

\newcommand{\BDM}[1]{\textrm{BDM}_{#1}}
\newcommand{\RT}[1] {\textrm{RT}_{#1}}
\newcommand{\RTz}   {\textrm{RT}_{0}}

%% ------------------------------------------------------------------------------------------
%%
%% MESH ITEMS
%%
%% ------------------------------------------------------------------------------------------

%% geometric items
\renewcommand{\P} {\textsf{P}}            % polyhedral element
\newcommand  {\F} {f}% {\textsf{f}}            % polygonal  face
\newcommand  {\E} {e}% {\textsf{e}}            % edge
\newcommand  {\V} {v}% {\textsf{v}}            % vertex
\newcommand  {\T} {T}% {\textsf{T}}            % tetraedra/triangle
\renewcommand{\S} {\sigma} %%{\textsf{s}} % sides
\newcommand  {\Psgm}{\P_{\S}}

%% modified geometric symbols
% vertices
\newcommand{\Vt}  {\widetilde{\V}}
\newcommand{\Vp}  {\V_{1}}
\newcommand{\Vpp} {\V_{2}}

% edges
\newcommand{\Et}  {\widetilde{\E}}
\newcommand{\Ehat}{\hat{\E}}
\newcommand{\Ep}  {\E_{1}}
\newcommand{\Epp} {\E_{2}}

% faces
\newcommand{\Ft}  {\widetilde{\F}}
\newcommand{\Fhat}{\hat{\F}}
\newcommand{\Fp}  {\F_{1}}
\newcommand{\Fpp} {\F_{2}}

% polyhedrons
\newcommand{\Pt}  {\widetilde{\P}}
\newcommand{\Phat}{\HAT{\P}}
\newcommand{\Pp}  {\P_{1}}
\newcommand{\Ppp} {\P_{2}}

%% the mesh & mesh size
\newcommand{\hh}{h}
\newcommand{\Th}{\Omega_{\hh}}

%% barycenters
\newcommand{\xvP}{\xv_{\P}}        % element
\newcommand{\xvF}{\xv_{\F}}        % face
\newcommand{\xvE}{\xv_{\E}}        % edge
\newcommand{\xvV}{\xv_{\V}}        % vertex
\newcommand{\xvS}{\xv_{\S}}        % sides

%% general
\newcommand{\DIM} {d}              % space dimension
\newcommand{\INT} {0}              % space dimension
\newcommand{\BND} {\partial}       % space dimension

%% characteristic lengths
\newcommand{\hP}{\hh_{\P}}
\newcommand{\hF}{\hh_{\F}}
\newcommand{\hE}{\hh_{\E}}
\newcommand{\hT}{\hh_{\T}}
\newcommand{\hS}{\hh_{\S}}

%% measures
%% \newcommand{\mP}{\ABS{\P}}
%% \newcommand{\mF}{\ABS{\F}}
%% \newcommand{\mE}{\ABS{\E}}
%% \newcommand{\mT}{\ABS{\T}}
%% \newcommand{\mS}{\ABS{\S}}

%% sets
\newcommand{\Pset}{\mathcal{P}}    % mesh polyhedrons
\newcommand{\Fset}{\mathcal{F}}    % mesh faces
\newcommand{\Eset}{\mathcal{E}}    % mesh edges
\newcommand{\Vset}{\mathcal{V}}    % mesh nodes
\newcommand{\Sset}{\mathcal{S}}    % generic symbol

%% cardinalities,
\newcommand{\NMB}{N}
\newcommand{\NP}{\NMB^{\Pset}}   % cardinality of the set of polyhedrons
\newcommand{\NF}{\NMB^{\Fset}}   % cardinality of the set of faces
\newcommand{\NE}{\NMB^{\Eset}}   % cardinality of the set of edges
\newcommand{\NV}{\NMB^{\Vset}}   % cardinality of the set of vertices
\newcommand{\NS}{\NMB^{\Sset}}   % cardinality of the set of vertices

%% cardinalities,
\newcommand{\NPV}{\NMB^{\Vset}_{\P}}      % number of vertices of polyhedron P
\newcommand{\NPE}{\NMB^{\Eset}_{\P}}      % number of edges    of polyhedron P
\newcommand{\NPF}{\NMB^{\Fset}_{\P}}      % number of faces    of polyhedron P
\newcommand{\NFV}{\NMB^{\Vset}_{\F}}      % number of vertices of face F
\newcommand{\NFE}{\NMB^{\Eset}_{\F}}      % number of edges    of face F

%% ------------------------------------------------------------------------------------------
%%
%% OPERATORS
%%
%% ------------------------------------------------------------------------------------------

%% measures
\newcommand{\dL}{\,dL}
\newcommand{\dV}{\,dV}
\newcommand{\dS}{\,dS}
\newcommand{\dxv}{\,d\xv}

\newcommand{\dt}{dt}
\newcommand{\dx}{dx}
\newcommand{\dy}{dy}
\newcommand{\dz}{dz}

%% differential operators (continuous)
\newcommand{\GRAD} {\textbf{grad}\,}
\newcommand{\CURL} {\textbf{curl}\,}
\newcommand{\ROTv} {\textbf{rot}\,}
\newcommand{\ROTs} {\textrm{rot}\,}
\newcommand{\Curls}{\text{curl}_{\xiv}}
\newcommand{\Curlv}{\text{Curl}_{\xiv}}
\newcommand{\DIV}  {\text{div}\,}
\newcommand{\LAPL} {\Delta}

%% differential operators (discrete)
\newcommand{\GRADH}{\GRAD_{\hh}}
\newcommand{\CURLH}{\CURL_{\hh}}
\newcommand{\ROTH} {\ROT_{\hh}}
\newcommand{\DIVH} {\DIV_{\hh}}
\newcommand{\LAPLH}{\LAPL_{\hh}}

%% DUAL differential operators (continuous)
\newcommand{\dGRAD} {\mathrm{GRAD}}
\newcommand{\dCURL} {\mathrm{CURL}}
\newcommand{\dDIV}  {\mathrm{DIV}}

%% DUAL differential operators (discrete)
\newcommand{\dGRADH}{\dGRAD_{\hh}}
\newcommand{\dCURLH}{\dCURL_{\hh}}
\newcommand{\dDIVH} {\dDIV_{\hh}}

%% normal, tangential
\newcommand{\nor}  {\mathbf{n}}
\newcommand{\norE} {\mathbf{n}_{\E}}
\newcommand{\norF} {\mathbf{n}_{\F}}
\newcommand{\norP} {\mathbf{n}_{\P}}
\newcommand{\norS} {\mathbf{n}_{\S}}
\newcommand{\norPF}{\mathbf{n}_{\P,\F}}
\newcommand{\norPE}{\mathbf{n}_{\P,\E}}
\newcommand{\norFE}{\mathbf{n}_{\F,\E}}

\newcommand{\tng}  {\mathbf{t}}
\newcommand{\tngF} {\mathbf{t}_{\F}}
\newcommand{\tngE} {\mathbf{t}_{\E}}
\newcommand{\tngFE}{\mathbf{t}_{\F,\E}}
\newcommand{\tngPE}{\mathbf{t}_{\P,\E}} %% used by plates, chapter 12

%% ------------------------------------------------------------------------------------------
%%
%% FIELDS
%%
%% ------------------------------------------------------------------------------------------

%% scalar, f
\newcommand{\fsh}{\fs_{\hh}}

%% scalar, p
\newcommand{\psh}{\ps_{\hh}}
\newcommand{\psV}{\ps_{\V}}
\newcommand{\psE}{\ps_{\E}}
\newcommand{\psF}{\ps_{\F}}
\newcommand{\psP}{\ps_{\P}}
\newcommand{\psS}{\ps_{\S}}
\newcommand{\psI}{\ps_{\INTP}}
\newcommand{\psIP}{\ps_{\INTP}_{\P}}

%% scalar, q
\newcommand{\qsh}{\qs_{\hh}}
\newcommand{\qsV}{\qs_{\V}}
\newcommand{\qsE}{\qs_{\E}}
\newcommand{\qsF}{\qs_{\F}}
\newcommand{\qsP}{\qs_{\P}}
\newcommand{\qsS}{\qs_{\S}}
\newcommand{\qsI}{\qs_{\INTP}}
\newcommand{\qsIP}{\qs_{\INTP,\P}}

%% scalar, u
%% \newcommand{\uss} {\us^{s}}
\newcommand{\ussh}{\ush^{s}}
\newcommand{\ussht}{\widetilde{\us}_{\hh}^{s}}
\newcommand{\ush}{\us_{\hh}}
\newcommand{\usht}{\widetilde{\us}_{\hh}}
\newcommand{\usV}{\us_{\V}}
\newcommand{\usE}{\us_{\E}}
\newcommand{\usF}{\us_{\F}}
\newcommand{\usP}{\us_{\P}}
\newcommand{\usS}{\us_{\S}}
\newcommand{\usI}{\us_{\INTP}}
\newcommand{\usIP}{\us_{\INTP,\P}}

%% scalar, v
\newcommand{\vsh}{\vs_{\hh}}
\newcommand{\vshu}{\underline{\vs}_{\hh}}
\newcommand{\vsht}{\widetilde{\vs}_{\hh}}
\newcommand{\vsV}{\vs_{\V}}
\newcommand{\vsE}{\vs_{\E}}
\newcommand{\vsF}{\vs_{\F}}
\newcommand{\vsP}{\vs_{\P}}
\newcommand{\vsPt}{\widetilde{\vs}_{\P}}
\newcommand{\vsPF}{\vs_{\P,\F}}
\newcommand{\vsS}{\vs_{\S}}
\newcommand{\vsI}{\vs_{\INTP}}
\newcommand{\vsIP}{\vs_{\INTP,\P}}

%% scalar, w
\newcommand{\wsh}{\ws_{\hh}}
\newcommand{\wsht}{\widetilde{\ws}_{\hh}}
\newcommand{\wsV}{\ws_{\V}}
\newcommand{\wsE}{\ws_{\E}}
\newcommand{\wsF}{\ws_{\F}}
\newcommand{\wsP}{\ws_{\P}}
\newcommand{\wsS}{\ws_{\S}}
\newcommand{\wsI}{\ws_{\INTP}}
\newcommand{\wsIP}{\ws_{\INTP,\P}}

%% scalar, E
\newcommand{\Esh}{\Es_{\hh}}
\newcommand{\EsV}{\Es_{\V}}
\newcommand{\EsE}{\Es_{\E}}
\newcommand{\EsF}{\Es_{\F}}
\newcommand{\EsP}{\Es_{\P}}
\newcommand{\EsS}{\Es_{\S}}

%% scalar, B
\newcommand{\Bsh}{\Bs_{\hh}}
\newcommand{\BsV}{\Bs_{\V}}
\newcommand{\BsE}{\Bs_{\E}}
\newcommand{\BsF}{\Bs_{\F}}
\newcommand{\BsP}{\Bs_{\P}}
\newcommand{\BsS}{\Bs_{\S}}

%% scalar, F
\newcommand{\Fsh}{\Fs_{\hh}}
\newcommand{\FsV}{\Fs_{\V}}
\newcommand{\FsE}{\Fs_{\E}}
\newcommand{\FsF}{\Fs_{\F}}
\newcommand{\FsP}{\Fs_{\P}}
\newcommand{\FsS}{\Fs_{\S}}

%% scalar, G
\newcommand{\Gsh}{\Gs_{\hh}}
\newcommand{\GsV}{\Gs_{\V}}
\newcommand{\GsE}{\Gs_{\E}}
\newcommand{\GsF}{\Gs_{\F}}
\newcommand{\GsP}{\Gs_{\P}}
\newcommand{\GsS}{\Gs_{\S}}

%% scalar, H
\newcommand{\Hsh}{\Hs_{\hh}}
\newcommand{\HsV}{\Hs_{\V}}
\newcommand{\HsE}{\Hs_{\E}}
\newcommand{\HsF}{\Hs_{\F}}
\newcommand{\HsP}{\Hs_{\P}}
\newcommand{\HsS}{\Hs_{\S}}

%% vector, u
\newcommand{\uvh}{\uv_{\hh}}
\newcommand{\uvV}{\uv_{\V}}
\newcommand{\uvE}{\uv_{\E}}
\newcommand{\uvF}{\uv_{\F}}
\newcommand{\uvP}{\uv_{\P}}
\newcommand{\uvS}{\uv_{\S}}

%% vector, v
\newcommand{\vvh}{\vv_{\hh}}
\newcommand{\vvV}{\vv_{\V}}
\newcommand{\vvE}{\vv_{\E}}
\newcommand{\vvF}{\vv_{\F}}
\newcommand{\vvP}{\vv_{\P}}
\newcommand{\vvS}{\vv_{\S}}

%% vector, w
\newcommand{\wvh}{\wv_{\hh}}
\newcommand{\wvV}{\wv_{\V}}
\newcommand{\wvE}{\wv_{\E}}
\newcommand{\wvF}{\wv_{\F}}
\newcommand{\wvP}{\wv_{\P}}
\newcommand{\wvS}{\wv_{\S}}

%% vector, p
\newcommand{\pvI}{\pv_{\INTP}}
\newcommand{\pvh}{\pv_{\hh}}
\newcommand{\pvV}{\pv_{\V}}
\newcommand{\pvE}{\pv_{\E}}
\newcommand{\pvF}{\pv_{\F}}
\newcommand{\pvP}{\pv_{\P}}
\newcommand{\pvS}{\pv_{\S}}

%% vector, q
\newcommand{\qvI}{\qv_{\INTP}}
\newcommand{\qvh}{\qv_{\hh}}
\newcommand{\qvV}{\qv_{\V}}
\newcommand{\qvE}{\qv_{\E}}
\newcommand{\qvF}{\qv_{\F}}
\newcommand{\qvP}{\qv_{\P}}
\newcommand{\qvS}{\qv_{\S}}

%% vector, r
\newcommand{\rvI}{\rv_{\INTP}}
\newcommand{\rvh}{\rv_{\hh}}
\newcommand{\rvV}{\rv_{\V}}
\newcommand{\rvE}{\rv_{\E}}
\newcommand{\rvF}{\rv_{\F}}
\newcommand{\rvP}{\rv_{\P}}
\newcommand{\rvS}{\rv_{\S}}

%% vector, B
\newcommand{\Bvh}{\Bv_{\hh}}
\newcommand{\BvV}{\Bv_{\V}}
\newcommand{\BvE}{\Bv_{\E}}
\newcommand{\BvF}{\Bv_{\F}}
\newcommand{\BvP}{\Bv_{\P}}
\newcommand{\BvS}{\Bv_{\S}}

%% vector, E
\newcommand{\Evh}{\Ev_{\hh}}
\newcommand{\EvV}{\Ev_{\V}}
\newcommand{\EvE}{\Ev_{\E}}
\newcommand{\EvF}{\Ev_{\F}}
\newcommand{\EvP}{\Ev_{\P}}
\newcommand{\EvS}{\Ev_{\S}}

%% vector, F
\newcommand{\Fvh}{\Fv_{\hh}}
\newcommand{\FvV}{\Fv_{\V}}
\newcommand{\FvE}{\Fv_{\E}}
\newcommand{\FvF}{\Fv_{\F}}
\newcommand{\FvP}{\Fv_{\P}}
\newcommand{\FvS}{\Fv_{\S}}

%% vector, G
\newcommand{\Gvh}{\Gv_{\hh}}
\newcommand{\GvV}{\Gv_{\V}}
\newcommand{\GvE}{\Gv_{\E}}
\newcommand{\GvF}{\Gv_{\F}}
\newcommand{\GvP}{\Gv_{\P}}
\newcommand{\GvS}{\Gv_{\S}}

%% vector, H
\newcommand{\Hvh}{\Hv_{\hh}}
\newcommand{\HvV}{\Hv_{\V}}
\newcommand{\HvE}{\Hv_{\E}}
\newcommand{\HvF}{\Hv_{\F}}
\newcommand{\HvP}{\Hv_{\P}}
\newcommand{\HvS}{\Hv_{\S}}

%% vector, J
\newcommand{\Jvh}{\Jv_{\hh}}
\newcommand{\JvV}{\Jv_{\V}}
\newcommand{\JvE}{\Jv_{\E}}
\newcommand{\JvF}{\Jv_{\F}}
\newcommand{\JvP}{\Jv_{\P}}
\newcommand{\JvS}{\Jv_{\S}}

%% ------------------------------------------------------------------------------------------
%%
%% SCALAR PRODUCTS, NORMS, SEMIN-NORMS
%%
%% ------------------------------------------------------------------------------------------

%% exact bilinear forms
\newcommand{\asP}{\as^{\P}}
\newcommand{\bsP}{\bs^{\P}}
\newcommand{\csP}{\cs^{\P}}

%% discrete bilinear forms
\newcommand{\ash}{\as_{\hh}}
\newcommand{\bsh}{\bs_{\hh}}
\newcommand{\csh}{\cs_{\hh}}

\newcommand{\ashP}{\as^P_{\hh}}
\newcommand{\bshP}{\bs^P_{\hh}}
\newcommand{\cshP}{\cs^P_{\hh}}

\newcommand{\bsht} {\widetilde{\bs}_{\hh}}
\newcommand{\bshtP}{\widetilde{\bs}^{\P}_{\hh}}

\newcommand{\gD}{\gs_D}
\newcommand{\gN}{\gs_N}

\newcommand{\bilN} [2]{\left(#1,#2\right)_{\GamN}}
\newcommand{\bilNh}[2]{\left(#1,#2\right)_{\GamN,\hh}}

\newcommand{\scal} [1]{\left(#1\right)}
\newcommand{\scalP}[1]{\left(#1\right)_{\P}}
\newcommand{\scalV}[1]{\left(#1\right)_{\Vs}}
\newcommand{\scalVp}[1]{\left(#1\right)_{\Vsp}}
\newcommand{\scalW}[1]{\left(#1\right)_{\Ws}}

%% stabilization terms
\newcommand{\SP} {S^{\P}}
\newcommand{\SPt}{\widetilde{S}^{\P}}

%% norms and seminorms
\newcommand{\normh}[1]{\norm{#1}{1,\hh}} % Lorenzo's seminorm

\newcommand{\nlen}{\hspace{-0.2mm}}
\newcommand{\hskp}{\hspace{0.2mm}}

\newcommand{\snorm}  [2]{|#1|_{#2}}
\newcommand{\Snorm}  [2]{\Big|#1\Big|_{#2}}
\newcommand{\SNORM}  [2]{\left|#1\right|_{#2}}

\newcommand{\norm}   [2]{|\nlen|#1|\nlen|_{#2}}
\newcommand{\Norm}   [2]{\Big|\nlen\nlen\Big|\hskp #1\hskp\Big|\nlen\nlen\Big|_{#2}}
\newcommand{\NORM}   [2]{\left|\nlen\left|#1\right|\nlen\right|_{#2}}

\newcommand{\Tnorm}  [2]{|\nlen|\nlen|#1|\nlen|\nlen|_{{#2}}}
\newcommand{\TNorm}  [2]{\Big|\nlen\nlen\Big|\nlen\nlen\Big|\hskp #1\hskp\Big|\nlen\nlen\Big|\nlen\nlen\Big|_{#2}}
\newcommand{\TNORM}  [2]{\left|\nlen\left|\nlen\left|#1\right|\nlen\right|\nlen\right|_{{}_{#2}}}

%% abs, snorm, norm
\newcommand{\abs}    [1]{|#1|}
\newcommand{\Abs}    [1]{\Big|#1\Big|}
\newcommand{\ABS}    [1]{\left|#1\right|}

%% jumps
\newcommand{\jump}[1]{\lbrack\!\lbrack\,#1\,\rbrack\!\rbrack}

%% VEM spaces
\newcommand{\Vhk}{V^{\hh}_{k}}
\newcommand{\VhkP}{V_k(\P)}

%% monomial sets
\newcommand{\calMs}{\mathcal{M}^{*}}

%% projector (generic)
\newcommand{\Proj} {\Ps}
\newcommand{\Projs}{\Ps^{*}}

%% projectors
\newcommand{\Pin}[1]{\Pi^{\nabla}_{#1}}
\newcommand{\Piz}[1]{\Pi^{0}_{#1}}
\newcommand{\PiSz}[1]{\Pi^{0,\S}_{#1}}

\newcommand{\PiEz}[1]{\Pi^{0,\E}_{#1}}
\newcommand{\PiFz}[1]{\Pi^{0,\F}_{#1}}
\newcommand{\PiFn}[1]{\Pi^{\nabla,\F}_{#1}}

%% polynomials
%% \newcommand{\usp}{\us_{\pi}}
%% \newcommand{\vsp}{\vs_{\pi}}
%% \newcommand{\wsp}{\ws_{\pi}}

%%
\newcommand{\bscal}[1]{\langle #1 \rangle}

%% conformity error
\newcommand{\calNh}{\mathcal{N}_{\hh}}

%% constants
\newcommand{\cbot}{c_*}
\newcommand{\ctop}{c^*}
\newcommand{\cttop}{\widetilde{c}^*}
\newcommand{\ctbot}{\widetilde{c}_*}

\newcommand{\sumP}{\sum_{\P\in\Th}}

%% eqdef
\newcommand{\eqdef}{:=}
\newcommand{\defeq}{=:}

%% restrict
\newcommand{\restrict}[2]{{#1}_{|{#2}}}

\newcommand{\red}{\color{red}}

\newcommand{\EOD}{\end{document}}

\newcommand{\sfrac}[2]{\mbox{\scalebox{1.}{$\frac{#1}{#2}$}}}

\newcommand{\eigs}{\varepsilon}
\newcommand{\eigv}{\eigs}
\newcommand{\eigh}{\eigs_{\hh}}

\newcommand{\vphi}{\varphi}

\newcommand{\opT}{T}
\newcommand{\opTh}{T_{\hh}}

\newcommand{\PDh}{P_{\GDh}}

\newcommand{\bil}[2]{\langle#1,#2\rangle}

\newcommand{\SvP}{\Sv_{\P}}

\newcommand{\kb}{\bar{k}}

\newcommand{\rk}{r^{k}}

\newcommand{\rmin}{r_{min}}

\newcommand{\Ihk}{I^{\hh}_{k}}

\newcommand{\roundPrecision}{2}
\sisetup{round-mode=places, round-precision=\roundPrecision, tight-spacing=true, exponent-product=\cdot}


%%%%% Definition for the stabilization part
\newcommand{\bP} {\partial \P}            % boundary polyhedral element

\newcommand{\snorms}[2]{|#1|^2_{#2}}

\newcommand{\Nk}[1]{N_{#1}}
\newcommand{\Nkort}[1]{N_{#1}^{\bot}}
\newcommand{\ushat}{\widehat{\us}}
\newcommand{\shat}{\widehat{s}}
\newcommand{\stilde}{\widetilde{s}}
\newcommand{\utilde}{\widetilde{\us}}
\newcommand{\vtilde}{\widetilde{\vs}}

\newcommand{\Vhken}{V_{k,\text{en}}^h}
\newcommand{\Vhkaux}{V_{k,\text{aux}}^h}

%---------------------------------------------------------------
% COMANDI COLORE TESTO
\newcommand{\rosa}[1]{{\color{magenta} #1}} % magenta
\newcommand{\magenta}[1]{{\color{magenta} #1}} % magenta
\newcommand{\nero}[1]{{\color{black} #1}} % nero
\newcommand{\blu}[1]{{\color{blue} #1}} % blu
\newcommand{\rosso}[1]{{\color{red} #1}} %rosso
\newcommand{\verde}[1]{{\color{green} #1}} %verde

\long\def\COMMENT#1{{\color{red} \begin{comment} #1 \end{comment}}} %%
%\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
%\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\Real}{\mathbb R}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\BX}{\mathbf{B}(X)}

\newcommand{\llangle}{\langle\!\langle}
\newcommand{\rrangle}{\rangle\!\rangle}

\DeclareMathOperator{\fspan}{span}

\newcommand{\basis}{\mathfrak{B}}
\newcommand{\BaseQ}{\mathfrak{B}_Q}
\newcommand{\basf}{\phi}
\newcommand{\BaseU}{\mathfrak{B}_U}
\newcommand{\basv}{\psi}

\newcommand{\te}{\eta}
\newcommand{\ebase}{e}

%\newcommand{\V}{\mathcal V}
\newcommand{\Vh}{\mathcal V_h}

%\newcommand{\bil}{\frak{a}}
\newcommand{\A}{\mathfrak{A}}
%% \newcommand{\tW}{W^*}

\newcommand{\bpi}{\tilde \pi}
\newcommand{\D}{D}
\newcommand{\normP}{{\beta^{-1}}}

\newcommand{\dualscal}[2]{(#1,#2)_{-1}}
\newcommand{\matr}[1]{\mathbf{#1}}

\newcommand{\astab}{a_{\gamma}}
\newcommand{\gstab}{g_{\gamma}}

\renewcommand{\c}{c}

\newcommand{\hag}{\widehat \bil_\gamma}
\newcommand{\hbg}{\widehat \beta_\gamma}

%\renewcommand{\langle}{\oldlangle}
%\renewcommand{\rangle}{\oldrangle}
%%\renewcommand{\vec}[1]{\vv{#1}}

% \newcommand{\Whk}{W^h_k}
\newcommand{\tsP}{\sigma^*_\P}
% \newcommand{\tsP}{ s^*_\P}
\newcommand{\basedofs}{\mathfrak B}
\newcommand{\Nbdofs}{k N}

\newcommand{\G}{\mathcal{G}}
\newcommand{\hG}{\widehat{\mathcal{G}}}

\newcommand{\gridauxP}{\mathcal{G}_\textbf{aux}(\bP)}
\newcommand{\hgridauxP}{\widehat{\mathcal{G}}_\textbf{aux}(\bP)}

\newcommand{\Const}{W_h}
\newcommand{\Lin}{\widetilde W_h}

\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\spa}{span}

\newcommand{\Qtilde}{\widetilde Q_h}
\newcommand{\Gl}{\widetilde G_\ell^*}

\newcommand{\DOFSuno}{(\textbf{D1})}
\newcommand{\DOFSdue}{(\textbf{D2})}

\newcommand{\SRuno}{{\textbf{(G1)}}}
\newcommand{\SRdue}{{\textbf{(G2)}}}
\newcommand{\SRtre}{{\textbf{(G3)}}}
\newcommand{\SRfour}{{\textbf{(G4)}}}
\newcommand{\SRfive}{{\textbf{(G5)}}}

\newcommand{\gdue}{\gamma_2}
\newcommand{\EdgesP}{\mathcal{E}_\P}
\newcommand{\gbP}{\gamma_{\bP}}
%% \newcommand{\tE}{\widetilde\E}

\newcommand{\constSteinbach}{c_0}
\newcommand{\tNk}[1]{\widetilde N_{#1}}
\newcommand{\sP}{\sigma_P}
\newcommand{\sPlin}{\widetilde\sigma^P}
\newcommand{\Baselin}{\widetilde{\mathfrak{B}}}
\newcommand{\tphi}{\widetilde{\phi}}
\newcommand{\dphi}{\widetilde{\lambda}}
\newcommand{\Basedual}{\mathfrak{B}}

\DeclareMathOperator{\dimension}{dim}

\newcommand{\ringVhkP}{\mathring{V}_k(\P)}

\newcommand{\portedge}{\pi^0_{\bP}}

\newcommand{\idx}{\ell}
\newcommand{\TT}{TT}
\newcommand{\FT}{FT}

%% added

\newcommand{\TTR}{TT}
\newcommand{\FTR}{FT}

\newcommand{\TTRANK}{\textrm{TT-rank}}

% \newcommand{\proof}{\begin{proof}}
%\newcommand{\ENDPROOF}{\end{proof}}


% color for the text written by Massimiliano Martinelli
\newcommand{\mm}[1]{\textcolor{blue}{#1}}

\newcommand{\xiv}{{\bm\xi}}
\newcommand{\zetav}{{\bm\zeta}}             
\newcommand{\betav}{{\bm\beta}}
\newcommand{\gammav}{{\bm\gamma}}

%% ---
\newcommand{\calXn}{\calX_{\ns}}
\newcommand{\calYn}{\calY_{\ns}}

\newcommand{\calXnt}{\widetilde{\calX}_{\ns}}

\newcommand{\Lsn}{\Ls_{\ns}}
\newcommand{\Lsnt}{\widetilde{\Ls}_{\ns}}
\newcommand{\LsnTT}{\Ls^{\TT{} }_{\ns}}

\newcommand{\fsn}{\fs_{\ns}}
\newcommand{\bsn}{\bs_{\ns}}

\newcommand{\fsnTT}{\fs_{\ns}^{\TT{}}}
\newcommand{\bsnTT}{\bs_{\ns}^{\TT{}}}

\newcommand{\PIPPO}{~\textbf{PIPPO-PIPPO-PIPPO}~}

\newcommand{\range}[1]{]#1]\phantom{[[}}

\newcommand{\RNDG}{\scalebox{0.9}{{\sf rndg}}}
\newcommand{\TTSVD}{\scalebox{0.9}{{\sf TT-SVD}}}
\newcommand{\cTT}{\mathbbm{TT}}
\newcommand{\toll}{\epsilon}

%% 
\newcommand{\tAss}[1]{\tA_{#1}}
\newcommand{\tRss}[1]{\tR_{#1}}
\newcommand{\tUss}[1]{\tU_{#1}}
\newcommand{\tZss}[1]{\tZ_{#1}}
\newcommand{\MAXVOL}{\scalebox{0.9}{{\sf MaxVol}}}

% Local Variables:
% mode: latex
% End:


==> matrix_D.tex <==
%% Hey Emacs, this is -*-latex-*-

\clearpage
\section*{Appendix: Additional material on spectral methods (to be removed)}

\noindent
$\bullet$ Let $\{\xss{i}\}_{i=0}^n$ be the Legendre-Gauss-Lobatto
points and $\{\lss{i}(\xs)\}_{i=0}^n$ be the associated Lagrange basis
functions.
%%
The differentiation matrix $\Ds = (d_{ij})_{i,j=0}^n$ is defined by:
%%
\begin{align}
  d_{ij} = \left.\frac{d}{dx}\lss{j}(x)\right|_{x=\xss{i}}, \qquad 0\leq i,j\leq n.
\end{align}

\medskip\noindent
$\bullet$
For Legendre-Gauss-Lobatto points, the explicit entries are:
\begin{align}
  d_{ij} = \begin{cases}
    \frac{\Pss{n}(\xss{i})}{(\xss{i}-\xss{j})\Pss{n}(\xss{j})} & \text{if } i\neq j, \\[1ex]
    -\sum_{k=0,k\neq i}^n d_{ik} & \text{if } i=j,
  \end{cases}
\end{align}
where $\Pss{n}$ is the Legendre polynomial of degree $n$.

\medskip\noindent
$\bullet$
The differentiation matrix $\Ds$ has entries:
\begin{align}
  d_{ij} = \begin{cases}
    \frac{\Pss{n}(\xss{i})}{(\xss{i}-\xss{j})\Pss{n}(\xss{j})} & \text{if } i\neq j, \\[1ex]
    -\sum_{k=0,k\neq i}^n d_{ik} & \text{if } i=j, \\[1ex]
    \frac{n(n+1)}{4} & \text{if } (i,j)=(0,0), \\[1ex]
    -\frac{n(n+1)}{4} & \text{if } (i,j)=(n,n).
  \end{cases}
\end{align}

\medskip\noindent
$\bullet$
Let's derive the entries $d_{ij}$ of the differentiation matrix
$\Ds$.
%%
By definition:
%%
\begin{align}
  d_{ij} = \left.\frac{d}{dx}\lss{j}(x)\right|_{x=\xss{i}}.
\end{align}
%%
\begin{itemize}
\item[(1)] First, recall that the Lagrange basis functions are:
  \begin{align}
    \lss{j}(x) = \prod_{k=0,k\neq j}^n \frac{x-\xss{k}}{\xss{j}-\xss{k}}
  \end{align}
  
\item[(2)] For $i\neq j$, applying the product rule:
  \begin{align}
    \frac{d}{dx}\lss{j}(x) &= \lss{j}(x)\sum_{k=0,k\neq
      j}^n \frac{1}{x-\xss{k}}
  \end{align}
  
\item[(3)] When evaluating at $x=\xss{i}$ (remember $i\neq j$), we
  have $\lss{j}(\xss{i})=0$, but one term in the sum becomes
  singular. We can use L'Hôpital's rule.

\item[(4)] For Legendre-Gauss-Lobatto points, we can use the
  relationship:
  \begin{align}
    \lss{j}(x) = \frac{(1-x^2)\Pss{n}'(x)}{n(n+1)(\xss{j}-x)\Pss{n}(\xss{j})}
  \end{align}

\item[(5)] Differentiating and evaluating at $x=\xss{i}$ leads to:
  \begin{align}
    d_{ij} = \frac{\Pss{n}(\xss{i})}{(\xss{i}-\xss{j})\Pss{n}(\xss{j})} \qquad\text{for }i\neq j
  \end{align}

\item[(6)] For the diagonal entries ($i=j$), we use the fact that the
  derivative of a constant is zero:
  \begin{align}
    \sum_{j=0}^n d_{ij} = 0
  \end{align}
%%
  Therefore:
  \begin{align}
  d_{ii} = -\sum_{j=0,j\neq i}^n d_{ij}
  \end{align}
\end{itemize}

\medskip\noindent
$\bullet$
For the corner cases, we need to consider that $\xss{0}=-1$ and
$\xss{n}=1$ are the endpoints of the Legendre-Gauss-Lobatto grid.
%%
\begin{itemize}
\item[(1)] For these points, we can use the explicit form of the
  Legendre polynomial $\Pss{n}(x)$:
  \begin{align}
    \Pss{n}(-1) &= (-1)^n \\
    \Pss{n}(1) &= 1
  \end{align}

\item[(2)] At $x=-1$ ($i=j=0$), using the formula for $d_{ij}$:
  \begin{align}
    d_{0j} &= \frac{\Pss{n}(-1)}{(-1-\xss{j})\Pss{n}(\xss{j})} \\
    &= \frac{(-1)^n}{(-1-\xss{j})\Pss{n}(\xss{j})}
  \end{align}

\item[(3)] The sum for the diagonal entry becomes:
  \begin{align}
    d_{00} &= -\sum_{j=1}^n d_{0j} \\
    &= -\sum_{j=1}^n \frac{(-1)^n}{(-1-\xss{j})\Pss{n}(\xss{j})} \\
    &= \frac{n(n+1)}{4}
  \end{align}
  
\item[(4)] Similarly, at $x=1$ ($i=j=n$):
  \begin{align}
    d_{nj} &= \frac{\Pss{n}(1)}{(1-\xss{j})\Pss{n}(\xss{j})} \\
    &= \frac{1}{(1-\xss{j})\Pss{n}(\xss{j})}
  \end{align}
  
\item[(5)] The diagonal entry becomes:
  \begin{align}
    d_{nn} &= -\sum_{j=0}^{n-1} d_{nj} \\
    &= -\sum_{j=0}^{n-1} \frac{1}{(1-\xss{j})\Pss{n}(\xss{j})} \\
    &= -\frac{n(n+1)}{4}
  \end{align}
\end{itemize}

\medskip\noindent
$\bullet$
The values $\frac{n(n+1)}{4}$ and $-\frac{n(n+1)}{4}$ can be proven
using properties of the Legendre polynomials and the fact that the
Legendre-Gauss-Lobatto points are symmetric about zero.
%%
Let's prove that $d_{00} = \frac{n(n+1)}{4}$ and $d_{nn} =
-\frac{n(n+1)}{4}$.
%%
\begin{itemize}
\item[(1)] First, recall key properties of Legendre polynomials:
  \begin{align}
    (1-x^2)\Pss{n}'(x) &= -n(n+1)\Pss{n}(x) + \alpha_n(x) \\
    \alpha_n(x) &= nx\Pss{n}(x) - n\Pss{n-1}(x)
  \end{align}
  
\item[(2)] At the Legendre-Gauss-Lobatto points $\{\xss{j}\}_{j=0}^n$:
  \begin{align}
    \Pss{n}'(\xss{j}) = 0 \quad\text{for}\quad j=1,\ldots,n-1
  \end{align}
  
\item[(3)] For the Lagrange basis functions:
  \begin{align}
    \lss{j}(x) = \frac{(1-x^2)\Pss{n}'(x)}{n(n+1)(x-\xss{j})\Pss{n}(\xss{j})}
  \end{align}

\item[(4)] Taking the derivative:
  \begin{align}
    \frac{d}{dx}\lss{j}(x) &= \frac{-2x\Pss{n}'(x) + (1-x^2)\Pss{n}''(x)}{n(n+1)(x-\xss{j})\Pss{n}(\xss{j})} \\
    &- \frac{(1-x^2)\Pss{n}'(x)}{n(n+1)(x-\xss{j})^2\Pss{n}(\xss{j})}
  \end{align}

\item[(5)] For $x=-1$ ($\xss{0}$):
  \begin{align}
    \Pss{n}(-1) &= (-1)^n \\
    \Pss{n}'(-1) &= \frac{n(n+1)}{2}(-1)^{n-1}
  \end{align}
  
\item[(6)] Substituting these values and using L'Hôpital's rule:
  \begin{align}
    d_{00} &= \lim_{x\to-1} \frac{d}{dx}\lss{0}(x) \\
    &= \frac{n(n+1)}{4}
  \end{align}
  
\item[(7)] Similarly, for $x=1$ ($\xss{n}$):
  \begin{align}
    \Pss{n}(1) &= 1 \\
    \Pss{n}'(1) &= \frac{n(n+1)}{2}
  \end{align}
  
\item[(8)] Leading to:
  \begin{align}
    d_{nn} &= \lim_{x\to1} \frac{d}{dx}\lss{n}(x) \\
    &= -\frac{n(n+1)}{4}
  \end{align}
  The symmetry of these values reflects the symmetry of the
  Legendre-Gauss-Lobatto points about $x=0$.
\end{itemize}

\medskip\noindent
$\bullet$
For a differential problem with Dirichlet boundary conditions:
\begin{align}
  \begin{cases}
    \frac{d}{dx}u(x) = f(x), & x\in(-1,1) \\
    u(-1) = \alpha, & \text{(left boundary condition)} \\
    u(1) = \beta, & \text{(right boundary condition)}
  \end{cases}
\end{align}
%%
The modification follows these steps:
%%
\begin{itemize}
\item[(1)] First, we remove the rows corresponding to the boundary
  points (rows 0 and n) and replace them with the boundary conditions:
  \begin{align}
    \tilde{\Ds} = \begin{pmatrix}
      1 & 0 & 0 & \cdots & 0 \\
      d_{10} & d_{11} & d_{12} & \cdots & d_{1n} \\
      \vdots & \vdots & \vdots & \ddots & \vdots \\
      d_{n-1,0} & d_{n-1,1} & d_{n-1,2} & \cdots & d_{n-1,n} \\
      0 & 0 & 0 & \cdots & 1
    \end{pmatrix}
  \end{align}
  
\item[(2)] The corresponding right-hand side vector is modified as:
  \begin{align}
    \tilde{\bs} = \begin{pmatrix}
      \alpha \\
      f(\xss{1}) \\
      \vdots \\
      f(\xss{n-1}) \\
      \beta
    \end{pmatrix}
  \end{align}
  
\item[(3)] The linear system becomes:
  \begin{align}
    \tilde{\Ds}\,\us = \tilde{\bs}
  \end{align}

\end{itemize}

\medskip\noindent
$\bullet$
This modification ensures that:
%%
\begin{itemize}[nosep]
\item[-] The solution satisfies $u(-1) = \alpha$ and $u(1) = \beta$ exactly
\item[-] The differential equation is satisfied at the interior points
\item[-] The system remains well-conditioned
\end{itemize}

\medskip\noindent
$\bullet$
The spectral accuracy of the method is preserved under Dirichlet
boundary conditions, but with some important considerations:
%%
\begin{itemize}
\item[(1)] For a sufficiently smooth solution $u(x)$, the error in the
  spectral approximation follows:
  \begin{align}
  \|u - u_n\|_{\infty} \leq C N^{-m} \|u\|_{H^m},
  \end{align}
  where $m$ is related to the smoothness of the solution.

\item[2)] In particular, for an analytic solution, we maintain
  spectral (exponential) convergence:
  \begin{align}
    \|u - u_n\|_{\infty} \leq C e^{-\alpha N},
  \end{align}
  where $\alpha > 0$ depends on the width of the strip of analyticity of
  $u$ in the complex plane.

\item[(3)] However, if the boundary conditions are incompatible with
  the differential equation, meaning:
  \begin{align}
    \left.\frac{d}{dx}u(x)\right|_{x=-1} \neq f(-1) \quad\text{or}\quad 
    \left.\frac{d}{dx}u(x)\right|_{x=1} \neq f(1),
  \end{align}
  then boundary layers may appear, leading to:

  \begin{itemize}[nosep]
  \item Gibbs-type phenomena near the boundaries
  \item Deterioration of the convergence rate to algebraic order
  \item Potential oscillations that propagate into the interior
  \end{itemize}
  
\item[(4)] To maintain spectral accuracy, the solution should satisfy:
  \begin{align}
    u \in C^{\infty}[-1,1] \quad\text{and}\quad 
    \text{compatibility conditions at the boundaries}
  \end{align}
  
\item[(5)] The modified system remains well-conditioned because:
  \begin{itemize}
  \item The boundary rows have condition number 1
  \item The interior rows maintain their spectral properties
  \item The system is no longer singular
  \end{itemize}
\end{itemize}

\medskip\noindent
$\bullet$
Let's analyze the local convergence near boundaries through several
key aspects:
%%
\begin{itemize}
\item[(1)] First, we introduce the concept of boundary layer
  resolution. Near $x = \pm$, we can estimate the node spacing using
  the asymptotic behavior of Legendre-Gauss-Lobatto points:
  \begin{align}
    \Delta x_j \approx \frac{\pi^2}{2N^2} \quad\text{near boundaries}
  \end{align}

\item[(2)] For a solution with a boundary layer of thickness $\delta$,
  we need:
  \begin{align}
    \frac{\pi^2}{2N^2} \leq \delta
  \end{align}
  to resolve the layer adequately.

\item[(3)] The local error near boundaries can be analyzed using the
  weighted Sobolev norm:
  \begin{align}
    \|e\|_{W^{k,\infty}_{\omega}} = \max_{0\leq j\leq k} 
    \sup_{x\in[-1,1]} |\omega(x)D^je(x)|
  \end{align}
  where $\omega(x) = \sqrt{1-x^2}$ is the natural weight function.

\item[(4)] For an analytic function $u(x)$ with a boundary layer at x = -1:
  \begin{align}
    u(x) = u_s(x) + u_b\left(\frac{x+1}{\delta}\right)
  \end{align}
  where $u_s$ is smooth and $u_b$ is the boundary layer component.
  
\item[(5)] The local error estimate becomes:
  \begin{align}
    |u(x) - u_N(x)| &\leq C_1 e^{-\alpha N} \quad\text{away from boundaries} \\
    |u(x) - u_N(x)| &\leq C_2 N^{-k} \quad\text{near boundaries}
  \end{align}
  where $k$ depends on the compatibility conditions at the boundary.
  
\item[(6)] For incompatible boundary conditions, we can quantify the
  pollution effect:
  \begin{align}
    \|e\|_{\infty} \leq CN^{-1}\left(\sum_{j=0}^{k-1}
    \left|\frac{d^ju}{dx^j}(1) - \frac{d^ju_N}{dx^j}(1)\right|\right)
  \end{align}
  
\item[(7)] The resolution requirement for a boundary layer of
  thickness $\delta$ follows:
  \begin{align}
    N \geq C\sqrt{\frac{|\ln(\epsilon)|}{\delta}}
  \end{align}
  where $\epsilon$ is the desired accuracy.
\end{itemize}

% Local Variables:
% mode: latex
% End:


==> new_TTbgkc.tex <==
\paragraph{Background}
\label{subsec1:background}

\textcolor{cyan}{IN Nature family journal, i Methods sono una review ma "method" che permettono di ottenere i risultati riportati in "results". review per questi giornali. Questa sezione da rimuovere... The tensor-train (TT) format \cite{oseledets2011,oseledets2010a} is a
powerful mathematical construct, which effectively addresses the curse
of dimensionality through efficient storage schemes, was known in
quantum physics as \emph{Matrix Product States} (MPS)
\cite{schollwock2011density,verstraete2006matrix,vidal2003efficient,white1993density}
before being independently rediscovered in numerical mathematics
\cite{oseledets2009b,oseledets2011,oseledets2009new,oseledets2009recursive}.
%%
The TT framework implements \TTSVD{}~\cite{oseledets2011}, a
systematic decomposition algorithm yielding quasi-optimal
approximations with accuracy controlled through a tolerance parameter
$\epsilon$.
%%
Its natural compatibility with fundamental linear algebra operations,
supported by robust rank reduction procedures
\cite{verstraete2006matrix,oseledets2011}, makes it particularly
effective for PDE computations.
%%
The subsequent development of the quantized tensor train (QTT) format
\cite{khoromskij2011} enhanced the framework's capabilities through
dimensional quantization.
%%
The QTT approach particularly excels in identifying and exploiting
low-rank structures in discrete operators
\cite{oseledets2009a,oseledets2010b,Grasedyck2010,kazeev2012,kazeev2013b,khoromskij2018}.
%%
This advancement has sparked extensive research
\cite{Dolgov2012,kazeev2014,kazeev2018,bachmayr2020,khoromskij2011,kazeev2017,kazeev2022,kazeev2013a,markeeva2021}
across various PDE applications, with notable success in treating
elliptic PDEs exhibiting singularities and oscillatory behaviors
\cite{kazeev2018,bachmayr2020,khoromskij2011,kazeev2017,kazeev2022}.
%%
%% A significant enhancement came through advanced preconditioning
%% strategies, particularly the development of tensor-structured
%% Bramble-Pasciak-Xu (BPX) preconditioners
%% \cite{bramble1990parallel}.
%% %%
%% Initially proposed for uniformly elliptic
%% problems \cite{bachmayr2020} and later extended to singularly
%% perturbed cases \cite{khoromskij2018}, these techniques enable
%% efficient low-rank QTT representations on refined grids.
%%
The methodology has demonstrated remarkable versatility across PDE
categories, including second-order elliptic PDEs
\cite{kazeev2015,kazeev2018,khoromskij2011,kazeev2017,kazeev2022,khoromskij2018,markeeva2021},
the Helmholtz equation \cite{kazeev2017,fraschini2024a}, chemical
master equations \cite{kazeev2014,kazeev2015b}, molecular Schrödinger
equations \cite{kazeev2015}, and Fokker-Planck equations
\cite{Dolgov2012}.
%%
Recent applications extend to time-dependent incompressible
Navier-Stokes equations \cite{gourianov2022} and non-linear
Schrödinger equations using QTT-based multigrid renormalization
\cite{lubasch2018}.
}
%% OLD
\begin{comment}
The TT representation of multi-dimensional arrays
\cite{oseledets2011,oseledets2010a} is as a groundbreaking advancement
in high-dimensional data analysis and compression, fundamentally
transforming our approach to the computer treatment of complex
tensorial structures and the way we perform computations on them.
%%
This mathematical framework, which makes it possible to mitigate the
curse of dimensionality through its remarkable storage efficiency, was
known in quantum physics as the Matrix Product States (MPS)
\cite{schollwock2011density,verstraete2006matrix,vidal2003efficient,white1993density}.
%%
It was later rediscovered in numerical computing through pioneering
research
\cite{oseledets2009b,oseledets2011,oseledets2009new,oseledets2009recursive}.
%%
Its practical implementation features a systematic decomposition
algorithm for ``quasi-optimal'' approximations
\cite[Alg.~1]{oseledets2011}, offering user-controlled
accuracy-efficiency trade-off through a tolerance parameter
$\epsilon$.
%%
The framework's compatibility with fundamental linear algebraic
operations enhances its utility in designing efficient algorithms for
partial differential equations (PDEs).
%%
These computations are supported by robust rank reduction procedures
\cite{verstraete2006matrix,oseledets2011}.

The introduction of the quantized tensor train (QTT) format
\cite{khoromskij2011} further enhanced the standard TT approach
through the quantization of tensor dimensions.
%%
The QTT format excels in exploiting low-rank structures in discrete
operators
\cite{oseledets2009a,oseledets2010b,Grasedyck2010,kazeev2012,kazeev2013b,khoromskij2018},
a characteristic crucial for developing efficient tensor-based
numerical approximations to PDE solutions.
%% %%
%% When integrated with fine-grained low-order finite element methods,
%% the resulting QTT-FEM methodology provides a robust framework for
%% solving multidimensional PDEs while maintaining computational
%% efficiency.
%%
The past decade has witnessed extensive research
\cite{Dolgov2012,kazeev2014,kazeev2018,bachmayr2020,khoromskij2011,kazeev2017,kazeev2022,kazeev2013a,markeeva2021}
exploring various PDE applications.
%%
Studies of elliptic PDEs with singularities and high-frequency
oscillatory behaviors
\cite{kazeev2018,bachmayr2020,khoromskij2011,kazeev2017,kazeev2022}
have demonstrated exponential convergence rates comparable to hp-FEM
applications for singular solutions.
%%
Advanced preconditioning strategies have significantly enhanced the
framework's effectiveness.
%%
The development of tensor-structured preconditioners \emph{\`a la
Bramble-Pasciak-Xu} (BPX)~\cite{bramble1990parallel}, initially
proposed in \cite{bachmayr2020} for uniformly elliptic problems and
later extended to one-dimensional singularly perturbed scenarios
\cite{khoromskij2018}, enables efficient low-rank QTT representations
on highly refined grids, often eliminating the need for adaptive mesh
refinement.

The versatility of TT/QTT-based numerical methods spans diverse PDE
categories.
%%
Second-order elliptic PDEs have received substantial attention
\cite{kazeev2015,kazeev2018,khoromskij2011,kazeev2017,kazeev2022,khoromskij2018,markeeva2021},
alongside specialized investigations of the one-dimensional Helmholtz
equation \cite{kazeev2017,fraschini2024a}, chemical master equation
\cite{kazeev2014,kazeev2015b}, molecular Schrödinger equation
\cite{kazeev2015}, and Fokker-Planck equation
\cite{Dolgov2012}.
%%
Recent applications have expanded to include solutions for the
time-dependent incompressible Navier-Stokes equation for turbulent
structures \cite{gourianov2022} and the non-linear Schrödinger
equation using QTT-based multigrid renormalization \cite{lubasch2018}.
\end{comment}


==> sec51_new_spectral.tex <==
%% Hey Emacs, this is -*-latex-*-

\subsection*{Spectral Collocation Methods}

\medskip
\paragraph{Spectral approximations.}
Let $\calX$ and $\calY$ be suitable functional spaces.
%%
We consider a linear operator $\Ls:\calX\to\calY$ and, for
$\bs\in\calY$, we are interested in solving the problem
%%
\begin{align}
  \mbox{Find $\fs\in\calX$ such that:}\quad\Ls\,\fs = \bs.
  \label{eq:pblm:strong}
\end{align}
%%
The operator $\Ls$ can be rather generic, but for this
paper, we only examine applications in the framework of
transport-diffusion partial differential equations.
%%
In this case, formulation~\eqref{eq:pblm:strong} includes boundary and
initial conditions to be assigned to $\fs$.
%% , which can also be part of
%% the description of the functional spaces.
%%
We assume that problem~\eqref{eq:pblm:strong} is mathematically
well-posed in the sense of
Hadamard~\cite{Hadamard:1902}, and we numerically
discretize it through the spectral collocation method based on
algebraic polynomials.
%%
Spectral methods are a very effective tool in numerical
approximation of various mathematical models due to their excellent
convergence rate in the presence of very smooth
solutions~\cite{Funaro:1997,Canuto-Hussaini-Quarteroni-Zang:2007}.

%To ease the presentation and set up the ground for our 
%discussion, we start with a brief overview of the spectral collocation
%method in the \emph{one-dimensional case}.
%%
We express $\fs$ as a linear combination of $n+1$ basis functions
denoted by $\lss{i}(\xs)$, $0\leq\is\leq\ns$.
%%
These functions form a polynomial Lagrangian basis for a
predefined set of nodes $\vec{\xv}=\{\xss{j}\}_{j=0,1,\ldots,\ns}$ in
the computational domain, so that $\lss{i}(\xss{j})=\delta_{ij}$.
%%
The points $\xss{i}$ are the \emph{collocation points} and form the
\emph{collocation grid}.
%%
In this way, we will assume that
$\fs(\xs)\approx\fsn(\xs)=\sum_{0\le\is\le\ns}\fss{i}\ \lss{i}(x)$.
%%
As a consequence $\fsn \in \calXn$, where $\calXn$ is a finite
dimensional space.

In the examples to follow, the distribution of such nodes is not
uniform (i.e., with fixed mesh size).
%%
Indeed, we set $\xss{0}=-1$ and $\xss{\ns}=1$, and the remaining nodes
are the zeros of $\Pss{\ns}'$, which is the first derivative of the
$\ns$-th Legendre polynomial $\Pss{\ns}$.

In the pseudospectral method, equation~\eqref{eq:pblm:strong} is
required to be satisfied at the collocation nodes $\vec{\xv}$.
%we build $\Lsn$ and $\bsn$ by
%evaluating the operator $\Ls$ and the right-hand side term $\bs$ at
%the collocation points $\vec{\xv}$.
%%
To fix the idea, let us take $\Ls\eqdef\ds^2\slash{\dx^2}$ and let
$\lss{i}''$ be the second derivative of each element of the basis
function $\lss{i}$, for $i=0,1,\ldots,\ns$, so that
$\fsn''(\xs)=\sum_{0\le\is\le\ns}\fss{i}\ \lss{i}''(\xs)$
%%
(note that there is no approximation here since the second derivative
of a polynomial can be computed exactly).
%%
%Problem~\eqref{eq:pblm:discrete} is equivalent to 
We then build a corresponding linear system,
that, by choosing for instance $\ns=4$, takes the form:
%%
\begin{align}
  \big(\Lsn\fsn\big)(\vec{\xv})\eqdef
  {\underbrace{
      \BLK{
        \left[
          \begin{array}{ccccc}
            \lss{0}''(x_0)  & \lss{0}''(x_1) & \lss{0}''(x_2) & \lss{0}''(x_3) & \lss{0}''(x_4) \\[0.25em]
            \lss{1}''(x_0)  & \lss{1}''(x_1) & \lss{1}''(x_2) & \lss{1}''(x_3) & \lss{1}''(x_4) \\[0.25em]
            \lss{2}''(x_0)  & \lss{2}''(x_1) & \lss{2}''(x_2) & \lss{2}''(x_3) & \lss{2}''(x_4) \\[0.25em]
            \lss{3}''(x_0)  & \lss{3}''(x_1) & \lss{3}''(x_2) & \lss{3}''(x_3) & \lss{3}''(x_4) \\[0.25em]
            \lss{4}''(x_0)  & \lss{4}''(x_1) & \lss{4}''(x_2) & \lss{4}''(x_3) & \lss{4}''(x_4)
          \end{array}
          \right]}
    }_{\scalebox{0.8}{{$\phantom{XXXXXXXX}\Ds^2$}}}
  }
  %% ---
  \left[
    \begin{array}{c}
      \fsn(x_0) \\[0.25em] \fsn (x_1) \\[0.25em] \fsn (x_2) \\[0.25em] \fsn (x_3) \\[0.25em] \fsn (x_4)
    \end{array}
    \right] =
  %% ---
  \left[
    \begin{array}{c}
      \bs(x_0) \\[0.25em] \bs(x_1) \\[0.25em] \bs(x_2) \\[0.25em] \bs(x_3) \\[0.25em] \bs(x_4)
    \end{array}
    \right]
  \defeq \bs(\vec{\xv}).
  %% ---
  \label{eq:linear:system}
\end{align}
%
%
In Equation~\eqref{eq:linear:system}, the left-hand side matrix, called $\Ds^2$,
provides the spectral collocation discretization of the second
derivative operator $d^2\slash{\dx^2}$.
%%
The entries of such a matrix are constructed by
evaluating the second derivatives of each element of the Lagrange basis at the
collocation points.
%%
For a general $n$, we have that $D^2=\Lsn=\{\lss{i}''(\xss{j})\}$,
$i,j=0,1,\ldots,\ns$, is a $(\ns+1)\times(\ns+1)$ matrix.
%%
To impose Dirichlet boundary conditions, the first and the last row of
the above matrix will be forced to be the corresponding first and last
row of the $(\ns+1)\times(\ns+1)$ identity matrix.
%%
Furthermore, we impose the proper boundary conditions by suitably
replacing $\bs(x_0)$ and $\bs(x_4)=\bs(x_n)$.
%%
For example, we set $\bs(x_0)=\bs(x_n)=0$ in the homogeneous case.

The theory of stability and convergence of the spectral collocation
method dates back to the
70s~\cite{Gottlieb-Orszag:1977,Canuto-Hussaini-Quarteroni-Zang:2007}.
%% 70s~\cite{Gottlieb-Orszag:1977,Shen-Tang-Wang:2011,Hesthaven-Gottlieb-Gottlieb:2007,Canuto-Hussaini-Quarteroni-Zang:2007}.
%%
We briefly recall that stability requires the boundedness of the
approximate solution in some suitable norm.
%%
The bound must be uniform versus the discretization parameter $n$.
%%
As the consistency property is satisfied, i.e., exact and discretized
operators coincide in a suitable finite dimensional space, convergence
of $\fsn$ to $\fs$ is obtained in certain normed
spaces~\cite{Canuto-Hussaini-Quarteroni-Zang:2007}.
%%
The convergence, for spectral type approximations, displays an
exponential rate under the hypotheses of high regularity of the
solution~\cite{Maday-Quarteroni:1979}.
%%
This makes this numerical technique very competitive with other known
methods, as it requires far fewer degrees of freedom if the
regularity assumptions on the exact solution are fulfilled.

\medskip
\paragraph{Superconsistency.}
%%
To define a superconsistent method, we introduce a second grid of
$n-1$ points, e.g., $\vec{\zv}=\{\zss{j}\}_{j=1,\ldots,\ns -1}$,
within the computational domain, according to the following recipe.
%%
Hereafter, we will refer to the points $\xss{\is}$ introduced in the
previous section as the \emph{representation points}, and the points
$\zss{i}$ as the \emph{collocation points}.
%
Accordingly, we say that $\vec{\xv}$ is the \emph{representation
grid}, and $\vec{\zv}$ is the \emph{collocation grid}.
%%
We use the representation points to express $\fsn=\{ \fsn(x_i) \}$.
%%
Instead, we use the collocation points to derive the numerical method.
%%
The approximation still keeps the form introduced above,
%in~\eqref{eq:pblm:discrete}, 
but now we require that
$\Lsn(\fsn(\vec{\xv}))=\big(\Lsn\fsn\big)(\vec{\zv})=\bsn(\vec{\zv})$.
%%
Now $\Lsn$ transforms a vector built at the nodes
$\vec{\xv}$ into a vector built at the nodes $\vec{\zv}$.
%%
Thus, at the interior of the domain, the new set of points replaces
the old one, which is only used to express the approximated solution.
%%
In other words, we look for the values $\fsn(\vec{\xv})$, but we require the problem to be satisfied at the points $\vec{\zv}$.
%%
The two sets of points may coincide, but this depends on the operator
$\Ls$, to realize a specific property.
%%
The method is said to be \emph{superconsistent} if the following
consistency condition holds for a functional space $\calXnt$ larger
than $\calXn$:
%%
\begin{align}
  \big(\Ls\qs\big)(\vec{\zv}) = \Lsn\big(\qs(\vec{\xv})\big)
  \qquad\forall\qs\in\calXnt.
\end{align}
%%
This means that the exact operator applied to $\qs$ and successively
evaluated at $\vec{\zv}$, equals the discrete operator applied to the
same $\qs$ evaluated at the nodes $\vec{\xv}$.
%%
We want this to be true for functions that are outside the
approximation space $\calXnt$, realizing in this way a higher degree
of consistency.
%%
This construction can be done, in principle, for a large range of
problems, as, for example, the approximation of integral equations\cite{Funaro:2004}.

%\begin{example}
%%
Let $\calXnt=\calXn\cup\textrm{span}(\chi)$ and consider the
one-dimensional convection-diffusion operator
\begin{align*}
  \Ls\eqdef\beta\cdot \ds\slash{\dx} - \varepsilon\cdot\ds^2\slash{\dx^2}.
\end{align*}
%% As proposed in~\cite{Funaro-Fatone-Scannavini:2007} we choose
%%
We consider the function $\chi\eqdef\chi_{n+1}=(1-x^2)\,\Pss{n}'$,
where $\Pss{n}'$ is the first derivative of the Legendre polynomial
$\Pss{n}$ of degree $n$~\cite{Funaro-Fatone-Scannavini:2007}.
%%
Now, imposing the superconsistent condition amounts to determining the
points $\vec{\zv}$ in such a way that:
%%
\begin{align*}
  \ns(\ns+1)
  \left[
    \varepsilon\Pss{\ns}' - \beta\Pss{\ns}
    \right](\zss{j}) = 0\ \quad \mathrm{for}\,j=1,\ldots,\ns-1.
\end{align*}
%%
These points are located between the zeros of $\Pss{\ns}$ and
$\Pss{n}'$ and their location depends on the ratio between
$\varepsilon$ and $\beta$, as shown in Figure~\ref{fig:superc-1d}.

%\end{example}
%% To evaluate the operators on the superconsistent
%% collocation grid, we define $S_n$ as the interpolation matrix such that:
%% \[
%% S_n\, \vec{\xv}  =\vec{\zv}.
%% \]
%% The superconsistent discrete problem can be alternatively formulated in the following way:
%% \[
%% S_n\,L_n f_n = S_n\, b_n. 
%% \]

% Local Variables:
% mode: latex
% End:





==> sec53_new_TTmethod.tex <==
%% Hey Emacs, this is -*-latex-*-

\subsection*{\mymethod{} algorithm for convection-diffusion-reaction equations}
\label{subsec:MyMethod}

\medskip
%%
We consider the problem defined by \eqref{eq:pblm:time:A},
\eqref{eq:pblm:time:B}, and \eqref{eq:pblm:time:C} defined
on the $d$-dimensional hypercube $\Omega\subset\REAL^{d}$, with
boundary conditions $\partial\Omega$.
%%
Therein, $\varepsilon$ is the (scalar) diffusion coefficient,
$\betav=(\beta_{\ell})_{\ell=1,2,\ldots,d}$ is the $d$-sized
vector-valued convection field, $\rho$ is the scalar reaction
coefficient, $\bs$ is the right-hand side source term.
%%
The coefficients $\varepsilon$, $\betav$, and $\rho$ can be constant
or varying in space as a function of the multidimensional position
vector $\xv\in\REAL^{d}$.
%%
In the last case, we assume that these coefficients satisfy
appropriate regularity conditions so that
problem~\eqref{eq:pblm:time:A}-\eqref{eq:pblm:time:C} is well-posed.
%%
For example, we can assume that $(i)$ $\varepsilon(\xv)$ is
\emph{uniformly positive}, i.e., there exists a strictly positive
constant $\epsilon_0$ such that $\varepsilon(\xv)\geq\epsilon_0$ for
all $\xv\in\Omega$; $(ii)$ the components of $\betav$ are smooth
(e.g., at least $\beta_{\ell}\in\CS{1}(\Omega)$) and bounded; $(iii)$
$\rho$ is bounded and non-negative, i.e., $\rho\geq 0$.
%%
In such a case, we also assume that a sufficiently accurate, low-rank
representation in tensor train format exists for all non-constant
coefficients.
%%
If these coefficients are low-rank, we can obtain their TT
representation through an application of the cross-interpolation
algorithm.

\medskip
\paragraph{The discrete diffusion operator.}
%%
The low-rank, TT representation of $\varepsilon$ reads as
$\varepsilon^{\TT}=\varepsilon_{1}\bowtie\varepsilon_{2}\bowtie\ldots\bowtie
\varepsilon_{d}$, where the cores are given in the core notation by
\begin{align*}
  \varepsilon_{\ell} = 
  \left[
    \begin{array}{cccc}
      \varepsilon_{\ell}(1,:,1) & \varepsilon_{\ell}(1,:,2) & \cdots & \varepsilon_{\ell}(1,:,r_{\ell}) \\[0.25em]
      \varepsilon_{\ell}(2,:,1) & \varepsilon_{\ell}(2,:,2) & \cdots & \varepsilon_{\ell}(2,:,r_{\ell}) \\[0.25em]
      \vdots                   & \vdots                  & \ddots & \vdots                        \\[0.25em]
      \varepsilon_{\ell}(r_{\ell-1},:,1) & \varepsilon_{\ell}(r_{\ell-1},:,2) & \cdots & \varepsilon_{\ell}(r_{\ell-1},:,r_{\ell)}
    \end{array}
    \right],
  \,\,
  \ell=1,2,\ldots,\DIM.
\end{align*}
%%
Then, for $\alpha_{\ell-1}=1,2,\ldots,\rss{\ell-1}$ and
$\alpha_{\ell}=1,2,\ldots,\rss{\ell}$, we set
$\Ess{\ell}(\alpha_{\ell-1},:,:,\alpha_{\ell})=\text{diag}\big(\varepsilon_{\ell}(\alpha_{\ell-1},:,\alpha_{\ell})\big)$,
so that every $\Ess{\ell}(\alpha_{\ell-1},:,:,\alpha_{\ell})$ is a
two-dimensional, diagonal matrix with
$\varepsilon_{\ell}(\alpha_{\ell-1},:,\alpha_{\ell})$ along the
diagonal.
%%
Using such a notation, we rewrite $\varepsilon^{\TT}$ as $\calE^{\TT}=
\calE_{1}\bowtie\calE_{2}\bowtie\ldots\bowtie\calE_{d}$, where each core of this tensor-train representation is the block matrix
%%
\begin{align*}
  \calE_{\ell} = 
  \left[
    \begin{array}{cccc}
      \Ess{\ell}(1,:,:,1) & \Ess{\ell}(1,:,:,2) & \cdots & \Ess{\ell}(1,:,:,\rss{\ell}) \\[0.25em]
      \Ess{\ell}(2,:,:,1) & \Ess{\ell}(2,:,:,2) & \cdots & \Ess{\ell}(2,:,:,\rss{\ell}) \\[0.25em]
      \vdots              & \vdots              & \ddots & \vdots                       \\[0.25em]
      \Ess{\ell}(\rss{\ell-1},:,:,1) & \Ess{\ell}(\rss{\ell-1},:,:,2) & \cdots & \Ess{\ell}(\rss{\ell-1},:,:,\rss{\ell})
    \end{array}
    \right],
  \,\,         
  \ell=1,2,\ldots,d.
\end{align*}

\newcommand{\Dsh}[1]{\Delta^{n}_{#1}}
\newcommand{\calDsz}[2]{\partial_{#1}^{#2}}
%%
For $\ell=1,2,\ldots,\DIM$, we let
$\Iss{\ell}(\alpha_{\ell-1},:,:,\alpha_{\ell})\in\REAL^{\nss{\ell}\times\nss{\ell}}$
be the $\nss{\ell}\times\nss{\ell}$-sized identity matrix for all
$\alpha_{\ell-1}=1,2,\ldots,\rss{\ell-1}$ and
$\alpha_{\ell}=1,2,\ldots,\rss{\ell}$.
%%
Finally, let $\Dsh{\ell}$ be the one-dimensional discretization of the
partial second derivative $\partial^2\slash{\partial\xss{\ell}}$ along
the direction $\ell$, which also includes the boundary conditions.
%%
Precisely, $\Dsh{\ell}$ is the $\big((\ns+1)\times(\ns+1)\big)$-sized
matrix operator $\Ds^2$ introduced in the left-hand side of
Equation~\eqref{eq:linear:system}, suitably modified to take into
account the Dirichlet boundary conditions, where we recall that $\ns$
is the polynomial degree of the spectral collocation approximation.
%%
Then, we consider the following approximation
$\Delta\approx\calD:=\calD_{1}\bowtie\calD_{2}\bowtie\ldots\bowtie\calD_{\DIM}$,
where each $\calD_{\ell}$ contains $\Dsh{\ell}$.
%%
%%, which is the spectral
%% collocation approximation of the second derivative, i.e., the matrix
%% operator $\Ds^2$, in the $\ell$-th direction, suitably modified to
%% include the boundary conditions.
%%
The cores $\calD_{\ell}$ are given by:
%%
\begin{align*}
  \calD_1 = 
  \left[
    \begin{array}{ccccc}
      \Dsh{1}(1,:,:,1) &  \Iss{1}(1,:,:,2) & \cdots & \Iss{1}(1,:,:,d-1)  & \Iss{1}(1,:,:,d) 
    \end{array}
    \right],
\end{align*}
%%
\begin{align*}
  \calD_{\ell} =
  \left[
    \begin{array}{ccccccc}
      {} \Iss{\ell}(1,:,:,1) &                     &         &                           &         &                         & \\
      {}                     & \Iss{\ell}(2,:,:,2) &         &                           &         &                         & \\
      {}                     &                     & \ddots  &                           &         &                         & \\
      {}                     &                     &         & \Dsh{\ell}(\ell,:,:,\ell) &         &                         & \\
      {}                     &                     &         &                           & \ddots  &                         & \\
      {}                     &                     &         &                           &         & \Iss{\ell}(d-1,:,:,d-1) & \\
      {}                     &                     &         &                           &         &                         & \Iss{\ell}(d,:,:,d)
    \end{array}
    \right],
\end{align*}

\begin{align*}
  \calD_{\DIM} = 
  \left[
    \begin{array}{c}
      \Iss{\DIM}(1,:,:,1)      \\
      \Iss{\DIM}(2,:,:,1)      \\
      \vdots                \\
      \Iss{\DIM}(d-1,:,:,1)\\
      \Dsh{\DIM}(d,:,:,1)
    \end{array}
    \right].
\end{align*}
%%
Finally, we consider the approximation
$\varepsilon\Delta\approx\calE\bowtie\calD$, where the cores of the
tensor train representation of $\calE\bowtie\calD$ are such that
$(\calE\bowtie\calD)_{\ell}=\calE_{\ell}\otimes\calD_{\ell}$ for
$\ell=1,2,\ldots,\DIM$.

\newcommand{\calNsz}[2]{\calN_{#1}^{#2}}

\medskip
\paragraph{The discrete convection operator.}

A similar reasoning can be applied to the first-order differential
operator $\betav\cdot\nabla$, where now $\betav$ is a vector
coefficient with $\DIM$ components, i.e.,
$\betav=\big(\beta_{1},\beta_{2},\ldots,\beta_{\DIM}\big)^T$, and the
partial differential operator $\nabla$ has also $\DIM$ components,
i.e., $\nabla=(\partial_1,\partial_2,\dots,\partial_{\DIM})^T$ with
the abbreviation $\partial_{\ell}=\partial\slash{\partial\xss{\ell}}$.
%%
We construct a tensor train representation of $\betav\cdot\nabla$ by
splitting the directional derivative along $\betav$ into its
directional components and then introducing the tensor train
representation of each term:
\begin{align*}
  \betav\cdot\nabla
  =      \sum_{\ell=1}^{\DIM}\beta_{\ell}\partial_{\ell}
  \approx\sum_{\ell=1}^{\DIM}\beta^{TT}_{\ell}\partial^{TT}_{\ell}
  = \betav^{TT}\cdot\nabla^{TT},
\end{align*}
or, equivalently, by saying that
$(\betav\cdot\nabla)^{TT}=\betav^{TT}\cdot\nabla^{TT}$, where
$\betav^{TT}=\big(\beta^{TT}_{1},\beta^{TT}_{2},\ldots,\beta^{TT}_{\DIM}\big)$
and
$\nabla^{TT}=(\partial^{TT}_1,\partial^{TT}_2,\dots,\partial^{TT}_{\DIM})$.
%%
Then, we build again the tensor train decomposition of each ``beta''
term as
$\beta^{TT}_{\ell}=\calB^{(\ell)}_{1}\bowtie\calB^{(\ell)}_{2}\bowtie\ldots\bowtie\calB^{(\ell)}_{\DIM}$
using the cores $\calB^{(\ell)}_{\ell'}$ and the tensor train
decomposition of the directional derivatives as
$\partial^{TT}_{\ell}=\calNsz{1}{(\ell)}\bowtie\calNsz{2}{(\ell)}\bowtie\ldots\calNsz{\DIM}{(\ell)}\bowtie$
using the cores $\calNsz{\ell'}{(\ell)}$.
%%
Using such an expansion on the cores, we finally found that
$\big(\beta^{TT}_{\ell}\bowtie\partial^{TT}_{\ell}\big)_{\ell'}=\calB^{(\ell)}_{\ell'}\otimes\calNsz{\ell'}{(\ell)}$,
which are the cores of each term
$\beta^{TT}_{\ell}\partial^{TT}_{\ell}$.
%%
To complete such a construction, we are just left to define the cores
$\calB^{(\ell)}_{\ell'}$ and $\calNsz{\ell'}{(\ell)}$.

The cores $\calB_{\ell,\ell'}$ are given by:
%%
\begin{align*}
  \calB^{(\ell)}_{\ell'} = 
  \left[
    \begin{array}{cccc}
      \Bsz{\ell'}{(\ell)}(1,:,:,1)                     & \Bsz{\ell'}{(\ell)}(1,:,:,2)                     & \cdots & \Bsz{\ell'}{(\ell)}(1,:,:,\rsz{\ell'}{(\ell)}) \\[0.5em]
      \Bsz{\ell'}{(\ell)}(2,:,:,1)                     & \Bsz{\ell'}{(\ell)}(2,:,:,2)                     & \cdots & \Bsz{\ell'}{(\ell)}(2,:,:,\rsz{\ell'}{(\ell)}) \\[0.5em]
      \vdots                                           & \vdots                                           & \ddots & \vdots                                         \\[0.5em]
      \Bsz{\ell'}{(\ell)}(\rsz{\ell'-1}{(\ell)},:,:,1) & \Bsz{\ell'}{(\ell)}(\rsz{\ell'-1}{(\ell)},:,:,2) & \cdots & \Bsz{\ell'}{(\ell)}(\rsz{\ell'-1}{(\ell)},:,:,\rsz{\ell'}{(\ell)})
    \end{array}
    \right],
\end{align*}
%%
where $\rsz{\ell'}{(\ell)}$ is the $\ell'$-th rank of the TT
decomposition of $\beta^{TT}_{\ell}$, and, for consistency it holds
that $\rsz{0}{(\ell)}=\rsz{\DIM}{(\ell)}=1$.

To build $\calNsz{\ell'}{(\ell)}$, we first denote by
$\calDsz{\ell}{n}$ the (matrix) operator representing the
one-dimensional partial derivative along the direction $\ell$ that is
provided by the spectral collocation discretization.
%%
We also denote by $\Isz{\ell'}{(\ell')}$ the four-dimensional tensor
with size
$\rsz{\ell'-1}{(\ell)}\times\nss{\ell'}\times\nss{\ell'}\times\rsz{\ell'}{(\ell)}$
such that the slice
$\Isz{\ell'}{(\ell)}(\alpha_{\ell'-1},:,:,\alpha_{\ell'})$ is the
identity matrix with size $(\nss{\ell'}\times\nss{\ell'})$ for all
admissible values of $\alpha_{\ell'-1}$ and $\alpha_{\ell'}$.
%%
Then, $\calNsz{\ell'}{(\ell')}$ for all $\ell$ is given by
%%
\begin{align*}
  \calNsz{1}{(\ell)} = 
  \left[
    \begin{array}{ccccc}
      \calDsz{1}{n}(1,:,:,1) &  \Isz{1}{(\ell)}(1,:,:,2) & \cdots & \Isz{1}{(\ell)}(1,:,:,d-1)  & \Isz{1}{(\ell)}(1,:,:,d) 
    \end{array}
    \right],
\end{align*}

\begin{align*}
  \calNsz{\ell'}{(\ell')} = 
    \left[
      \begin{array}{cccccc}
        {} \Isz{\ell'}{(\ell)}(1,:,:,1) &                              &         &                                  &                                   & \\
        {}                              & \Isz{\ell'}{(\ell)}(2,:,:,2) &         &                                  &                                   & \\
        {}                              &                              & \ddots  &                                  &                                   & \\
        {}                              &                              &         & \calDsz{\ell'}{n}(\ell,:,:,\ell) &                                   & \\
        {}                              &                              &         &                                  & \ddots                            & \\
        {}                              &                              &         &                                  & \Isz{\ell'}{(\ell)}(d-1,:,:,d-1)  & \\
        {}                              &                              &         &                                  &                                   & \Isz{\ell'}{(\ell)}(\DIM,:,:,\DIM)
      \end{array}
      \right],\,\,
    \ell'=2,\ldots,\DIM-1,
\end{align*}

\begin{align*}
  \calNsz{\DIM}{(\ell)} = 
  \left[
    \begin{array}{c}
      \Isz{\DIM}{(\ell)}(1,:,:,1)      \\
      \Isz{\DIM}{(\ell)}(2,:,:,1)      \\
      \vdots                           \\
      \Isz{\DIM}(d-1,:,:,1)            \\
      \calDsz{\DIM}{n}(d,:,:,1)
    \end{array}
    \right].
\end{align*}

\medskip
\paragraph{The discrete reaction operator.}
%%
Following the same approach used for the diffusion and convection
operators, we now construct the discrete reaction operator in tensor
train format.
%%
The low-rank, TT representation of $\rho$ reads as
$\rho^{\TT}=\rho_{1}\bowtie\rho_{2}\bowtie\ldots\bowtie\rho_{d}$,
where the cores are given in the core notation by
\begin{align*}
  \rho_{\ell} = 
  \left[
    \begin{array}{cccc}
      \rho_{\ell}(1,:,1)        & \rho_{\ell}(1,:,2)        & \cdots & \rho_{\ell}(1,:,r_{\ell}) \\[0.25em]
      \rho_{\ell}(2,:,1)        & \rho_{\ell}(2,:,2)        & \cdots & \rho_{\ell}(2,:,r_{\ell}) \\[0.25em]
      \vdots                   & \vdots                   & \ddots & \vdots                 \\[0.25em]
      \rho_{\ell}(r_{\ell-1},:,1) & \rho_{\ell}(r_{\ell-1},:,2) & \cdots & \rho_{\ell}(r_{\ell-1},:,r_{\ell)}
    \end{array}
    \right],
  \,\,
  \ell=1,2,\ldots,\DIM.
\end{align*}
%%
Then, we introduce the reaction term $\calR$, which is
represented through the core sequence
$\calR^{\TT}=\calR_{1}\bowtie\calR_{2}\bowtie\ldots\bowtie\calR_{d}$,
where each core corresponds to a spatial dimension.
%%
The $\ell$-th core is given by
%%
\begin{align*}
  \calR_{\ell} = 
  \left[
    \begin{array}{cccc}
      \Rss{\ell}(1,:,:,1) & \Rss{\ell}(1,:,:,2) & \cdots & \Rss{\ell}(1,:,:,\rss{\ell}) \\[0.25em]
      \Rss{\ell}(2,:,:,1) & \Rss{\ell}(2,:,:,2) & \cdots & \Rss{\ell}(2,:,:,\rss{\ell}) \\[0.25em]
      \vdots              & \vdots              & \ddots & \vdots                       \\[0.25em]
      \Rss{\ell}(\rss{\ell-1},:,:,1) & \Rss{\ell}(\rss{\ell-1},:,:,2) & \cdots & \Rss{\ell}(\rss{\ell-1},:,:,\rss{\ell})
    \end{array}
    \right],
  \,\,         
  \ell=1,2,\ldots,\DIM, 
\end{align*}
%%
where, for $\alpha_{\ell-1}=1,2,\ldots,\rss{\ell-1}$ and
$\alpha_{\ell}=1,2,\ldots,\rss{\ell}$, we set
$\Rss{\ell}(\alpha_{\ell-1},:,:,\alpha_{\ell})=\text{diag}(\rho_{\ell}(\alpha_{\ell-1},:,\alpha_{\ell})$,
so that every $\Rss{\ell}(\alpha_{\ell-1},:,:,\alpha_{\ell})$ is a
two-dimensional, diagonal matrix with
$\rho_{\ell}(\alpha_{\ell-1},:,\alpha_{\ell})$ along the
diagonal.
%%
Finally, we note that the diagonal structure of the matrices reflects
the multiplicative nature of the reaction term.

\medskip
\paragraph{The space-time formulation.}

\medskip
The final space-time differential operator includes the time
derivative term:
\begin{align*}
  \Lsn \eqdef
  \Dss{t}\otimes_{\ell=1}^{d}\Iss{\ell} +
  \Iss{t}\otimes
  \bigg[ -\calE\bowtie\calD + \sum_{\ell=1}^{d}\calB_{\ell}\bowtie\calN_{\ell} 
  + \calR
  \bigg],
\end{align*}
where $\Dss{t}$ e $\Iss{t}$ are the discrete derivative and the
identity matrix relative to the time discretization, where the time
operator is the approximation of $\partial\slash{\partial\ts}$.
%%
The superconsistent version of the scheme is achieved by evaluating
the terms $\calB$, $\calE$ and $\calR$ on the superconsistent grid.
%%
%% The operator $\Ds^{2}$ is corrected to $S_n\, \Ds^2$ in expression
%% (\ref{eq:tt-discrete-diffusion}) and the operator $\Ds$ is corrected
%% to $S_n\, \Ds$ in expression (\ref{eq:tt-discrete-advection}).
%% %%
%% Alternatively, defining $S_\ell$ the interpolation matrix along the
%% $\ell$-th direction, we can write:
%% \[
%% \calS = \Iss{t}\otimes_{\ell=1}^{d}S_{\ell}.
%% \]
%% The superconsistent operator can be evaluated as:
%% \begin{align*}
%%   \Lsn \eqdef \calS \cdot\left\{
%%   \Dss{t}\otimes_{\ell=1}^{d}\Iss{\ell} +
%%   \Iss{t}\otimes
%%   \bigg[ -\calE\cdot\calD^2 + \sum_{\ell=1}^{d}\calB_{\ell}\cdot\calN_{\ell} 
%%   + \calR
%%   \bigg]\right\}.
%% \end{align*}
%% Finally, the right-hand side is evaluated at the superconsistent
%% points.

% Local Variables:
% mode: latex
% End:


==> sec5_methods.tex <==
%% Hey Emacs, this is -*-latex-*-

\section*{Methods}
\label{sec5:methods}

In this section, we provide a formal mathematical description of the
\mymethod\ scheme.
We introduce the one-dimensional operators in the subsection ``Spectral Collocation Methods’’. 
Next, in section ``Tensor Train representation’’ we 
introduce the TT linear algebra format. 
Finally, in the section ``\mymethod algorithm for convection-diffusion-reaction equation’’ 
we present how the building blocks are integrated to construct 
the high-dimensional solver. 
%%
%We first introduce the spectral collocation
%method~\cite{Canuto-Hussaini-Quarteroni-Zang:2007} and its superconsistent
%formulation~\cite{Funaro:2002}, suited to the numerical resolution of
%advection-dominated transport problems~\cite{Funaro:1997}.
%%
%Then, we briefly review the main concepts about
%the tensor-train format and decompositions~\cite{Oseledets:2011}.
%%
%Finally, we discuss how to combine these elements to create an
%accurate, effective, and computationally efficient strategy for
%solving high-dimensional transport equations.%

\input{sec51_new_spectral.tex}
\input{sec52_new_TTformat.tex}
\input{sec53_new_TTmethod.tex}

% Local Variables:
% mode: latex
% End:


==> sec6_conclusions.tex <==
%% Hey Emacs, this is -*-latex-*-

\section*{Conclusions}
\label{sec6:conclusions}

\MGT{Possiamo fonderle con la section Discussion e eliminarle da qui (no problem).}
\textcolor{cyan}{Le conclusioni non sono richieste nel formato del giornale, anzi non dovrebbero essere scritte, il body del testo finisce con Discussion e poi iniziano i Methods}

This paper introduced \mymethod, a novel numerical solver that effectively addresses long-standing challenges \textcolor{blue}{esagerato} in solving high-dimensional transport equations.

The key contributions of this work can be summarized as follows. 
%%
First, with unprecedented speed, \mymethod enables the efficient solution of six-plus-time dimensional transport problems described by partial differential equations (PDEs). 
%%
Our numerical experiments demonstrate that problems requiring millions of years on current supercomputers \textcolor{blue}{moderare i termini} can be solved in minutes on standard computing hardware while maintaining accuracy to machine precision. 
%%
Second, as part of \mymethod, we extend the superconsistent approach to high-dimensional settings through a dimension-wise implementation that preserves stability across all parameter ranges. 
%%
This is particularly crucial in advection-dominated scenarios, where traditional methods typically fail. 
%%
Our tests confirm that \mymethod remains stable even for extremely small diffusion 
coefficients $\varepsilon\approx\mathcal{O}(10^{-12})$,
% (ε ≈ 10⁻⁶), 
accurately capturing boundary and internal layers. 
%%
Third, \mymethod preserves the spectral accuracy of traditional spectral methods while operating in high dimensions. 
%%
The method exhibits exponential convergence rates that remain independent of the advection-diffusion ratio, as verified through extensive numerical testing, including challenging cases such as the traveling bump test and Hughes’ boundary layer problem.

These results establish \mymethod as a powerful tool for a wide range of applications in physics and engineering, particularly in modeling high-dimensional transport phenomena. 
%%
Technological advances are driving the development of next-generation nuclear technologies, including small modular reactors, advanced modular reactors, microreactors, and nuclear fusion systems. 
%%
These innovations require massive neutronic and fluid dynamics calculations for reactor design and the entire nuclear fuel cycle, including nuclear safeguards, nonproliferation, and security
\cite{ecp2025reports,iaea2025aris,international2024iaea,geist2024nondestructive,cavallini2023vanquishing}.
%%
We expect \mymethod to be a key enabler numerical solver in addressing these complex computational challenges.

Beyond nuclear applications, \mymethod has the potential to impact a wide range of fields requiring efficient, high-dimensional transport computations. Its ability to solve such problems on standard computing hardware makes it particularly valuable for practical applications with limited computational resources.

Future directions of this work include extending the \mymethod architecture to run efficiently on supercomputers, further expanding its applicability to large-scale scientific and engineering problems.
\textcolor{blue}{questa section Conclusions va rivista sulla base di cio' che ci
siamo gia' detti}

\begin{comment}
This paper has introduced \mymethod, a novel numerical solver that
effectively addresses the long-standing challenges in solving
high-dimensional transport equations.
%%
Our approach successfully combines three established methodologies:
Spectral Collocation for accuracy, Superconsistency for stability, and
Tensor Train format for computational efficiency.
%%
The key findings of our work can be summarized in three main
achievements.
%%
First, \mymethod{} can solve six-plus-time
dimensional problems with unprecedented efficiency.
%%
Our numerical experiments show that problems requiring millions of
years of computation time on current supercomputers can be solved in
minutes on standard computing hardware, achieving compression ratios
of $\mathcal{O}(10^{-12})$ while maintaining accuracy to machine
precision.
%%
Second, the superconsistent approach has been extended to higher
dimensional situations through a dimension-wise implementation that
preserves stability across all parameter regimes.
%%
This advancement is particularly significant in advection-dominated
scenarios where traditional methods typically fail.
%%
Our numerical tests confirm that \mymethod{} remains stable even with
extremely small diffusion coefficients ($\varepsilon\approx 10^{-6}$),
while accurately capturing both boundary and internal layers.
%%
Third, \mymethod{} preserves the spectral accuracy of traditional
spectral methods while operating in high dimensions.
%%
The method exhibits exponential convergence rates independent of the
advection-diffusion ratio, a property that has been verified through
extensive numerical testing, including challenging cases such as the
traveling bump test and Hughes' boundary layer problem.

These results establish \mymethod{} as a promising tool for a wide range of
applications in physics and engineering, particularly in fields such
as nuclear reactor design, plasma physics, and semiconductor modeling,
where high-dimensional transport phenomena play a crucial role.
%%
The method's ability to handle complex, multi-scale problems
efficiently on standard computing hardware makes it particularly
valuable for practical applications where computational resources are
limited.
%%
%% In our future work, we will explore the extension of \mymethod{} to
%% more general geometries through domain splitting and domain
%% decomposition, as well as its possible application to specific
%% industrial problems.
\end{comment}

% Local Variables:
% mode: latex
% End:


==> tt-blocks.tex <==
%Shape: Rectangle [id:dp7539563965485652] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (306,208) -- (354,208) -- (354,224) -- (306,224) -- cycle ;
%Straight Lines [id:da39901329352807036] 
\draw    (322,224) -- (322,208) ;
%Straight Lines [id:da16929740293146223] 
\draw    (338,224) -- (338,208) ;

%Shape: Rectangle [id:dp7204880880460114] 
\draw  [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ] (298,216) -- (346,216) -- (346,232) -- (298,232) -- cycle ;
%Straight Lines [id:da9467357929651048] 
\draw [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ]   (314,232) -- (314,216) ;
%Straight Lines [id:da6034769789875736] 
\draw [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ]   (330,232) -- (330,216) ;

%Shape: Rectangle [id:dp17001385766385213] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (290,224) -- (338,224) -- (338,240) -- (290,240) -- cycle ;
%Straight Lines [id:da04943542795879119] 
\draw    (306,240) -- (306,224) ;
%Straight Lines [id:da8340020117484499] 
\draw    (322,240) -- (322,224) ;

%Shape: Rectangle [id:dp4029095959688651] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (282,232) -- (330,232) -- (330,248) -- (282,248) -- cycle ;
%Straight Lines [id:da8931660690537624] 
\draw    (298,248) -- (298,232) ;
%Straight Lines [id:da5135391955056059] 
\draw    (314,248) -- (314,232) ;

%Shape: Rectangle [id:dp325198217034532] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (274,240) -- (322,240) -- (322,256) -- (274,256) -- cycle ;
%Straight Lines [id:da5623045877240891] 
\draw    (290,256) -- (290,240) ;
%Straight Lines [id:da5847978931965359] 
\draw    (306,256) -- (306,240) ;


%Shape: Rectangle [id:dp7581810853485804] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (215,192) -- (247,192) -- (247,240) -- (215,240) -- cycle ;
%Straight Lines [id:da3151032432784835] 
\draw    (215,208) -- (247,208) ;
%Straight Lines [id:da21700759476376397] 
\draw    (231,240) -- (231,192) ;
%Straight Lines [id:da8339475031733812] 
\draw    (215,224) -- (247,224) ;

%Shape: Rectangle [id:dp8059124123206534] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (207,200) -- (239,200) -- (239,248) -- (207,248) -- cycle ;
%Straight Lines [id:da9578409175621667] 
\draw    (207,216) -- (239,216) ;
%Straight Lines [id:da27177590083430014] 
\draw    (223,248) -- (223,200) ;
%Straight Lines [id:da6474025347749928] 
\draw    (207,232) -- (239,232) ;

%Shape: Rectangle [id:dp08365638710694356] 
\draw  [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ] (199,208) -- (231,208) -- (231,256) -- (199,256) -- cycle ;
%Straight Lines [id:da7049756067266619] 
\draw [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ]   (199,224) -- (231,224) ;
%Straight Lines [id:da6318866018278575] 
\draw [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ]   (215,256) -- (215,208) ;
%Straight Lines [id:da2453459703627816] 
\draw [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ]   (199,240) -- (231,240) ;

%Shape: Rectangle [id:dp6398721790720425] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (191,216) -- (223,216) -- (223,264) -- (191,264) -- cycle ;
%Straight Lines [id:da8045333994622963] 
\draw    (191,232) -- (223,232) ;
%Straight Lines [id:da11802535506570111] 
\draw    (207,264) -- (207,216) ;
%Straight Lines [id:da28963024630197265] 
\draw    (191,248) -- (223,248) ;


%Shape: Rectangle [id:dp3136498567080286] 
\draw  [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ] (150,200) -- (166,200) -- (166,232) -- (150,232) -- cycle ;
%Straight Lines [id:da7608892248073775] 
\draw [fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ]   (150,216) -- (166,216) ;

%Shape: Rectangle [id:dp2806215148435298] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (142,208) -- (158,208) -- (158,240) -- (142,240) -- cycle ;
%Straight Lines [id:da7970793518446402] 
\draw    (142,224) -- (158,224) ;

%Shape: Rectangle [id:dp19972434254476368] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (134,216) -- (150,216) -- (150,248) -- (134,248) -- cycle ;
%Straight Lines [id:da7030844496661988] 
\draw    (134,232) -- (150,232) ;


%Shape: Rectangle [id:dp771428895253814] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (50,168) -- (98,168) -- (98,248) -- (50,248) -- cycle ;
%Straight Lines [id:da027868198854172466] 
\draw    (50,184) -- (98,184) ;
%Straight Lines [id:da3385170199752563] 
\draw    (50,200) -- (98,200) ;
%Straight Lines [id:da3721655329204534] 
\draw    (50,232) -- (98,232) ;
%Straight Lines [id:da32753500935173974] 
\draw    (50,216) -- (98,216) ;
%Straight Lines [id:da09727967738624255] 
\draw    (66,248) -- (66,168) ;
%Straight Lines [id:da028618132895009918] 
\draw    (82,248) -- (82,168) ;

%Shape: Rectangle [id:dp7746751077373257] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (42,176) -- (90,176) -- (90,256) -- (42,256) -- cycle ;
%Straight Lines [id:da9861375826103267] 
\draw    (42,192) -- (90,192) ;
%Straight Lines [id:da9525148617004084] 
\draw    (42,208) -- (90,208) ;
%Straight Lines [id:da5138004478720457] 
\draw    (42,240) -- (90,240) ;
%Straight Lines [id:da6833395803096296] 
\draw    (42,224) -- (90,224) ;
%Straight Lines [id:da35030191614770567] 
\draw    (58,256) -- (58,176) ;
%Straight Lines [id:da16253791696791597] 
\draw    (74,256) -- (74,176) ;

%Shape: Rectangle [id:dp4262937400144504] 
\draw  [draw opacity=0][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (34,184) -- (82,184) -- (82,264) -- (34,264) -- cycle ;
%Shape: Rectangle [id:dp9956649334772427] 
\draw  [draw opacity=0][fill={rgb, 255:red, 32; green, 119; blue, 180 }  ,fill opacity=1 ] (66,200) -- (82,200) -- (82,216) -- (66,216) -- cycle ;
%Shape: Rectangle [id:dp6350796452437508] 
\draw   (34,184) -- (82,184) -- (82,264) -- (34,264) -- cycle ;
%Straight Lines [id:da7834751107267051] 
\draw    (34,216) -- (82,216) ;
%Straight Lines [id:da48087621532572444] 
\draw    (34,232) -- (82,232) ;
%Straight Lines [id:da8740972784869998] 
\draw    (66,264) -- (66,184) ;
%Straight Lines [id:da9753330189002731] 
\draw    (34,200) -- (82,200) ;

%Straight Lines [id:da6391576684937086] 
\draw    (50,264) -- (50,184) ;

%Straight Lines [id:da052602556705057424] 
\draw    (34,248) -- (82,248) ;

%Shape: Rectangle [id:dp950555129374252] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (26,192) -- (74,192) -- (74,272) -- (26,272) -- cycle ;
%Straight Lines [id:da35172027526573424] 
\draw    (26,208) -- (74,208) ;
%Straight Lines [id:da6129218590029197] 
\draw    (26,224) -- (74,224) ;
%Straight Lines [id:da07329199655400176] 
\draw    (26,256) -- (74,256) ;
%Straight Lines [id:da8989683874128502] 
\draw    (26,240) -- (74,240) ;
%Straight Lines [id:da17661474358360252] 
\draw    (42,272) -- (42,192) ;
%Straight Lines [id:da3595549571909642] 
\draw    (58,272) -- (58,192) ;

% Text Node
\draw (52,280) node [anchor=north][inner sep=0.75pt]    {$n_{1}$};
% Text Node
\draw (89,263) node [anchor=north west][inner sep=0.75pt]    {$n_{2}$};
% Text Node
\draw (100,205) node [anchor=north west][inner sep=0.75pt]    {$n_{3}$};
% Text Node
\draw (157,245) node [anchor=north west][inner sep=0.75pt]    {$n_{1}$};
% Text Node
\draw (142,254) node [anchor=north][inner sep=0.75pt]    {$r_{0}$};
% Text Node
\draw (175,211) node [anchor=north][inner sep=0.75pt]    {$r_{1}$};
% Text Node
\draw (210,268) node [anchor=north][inner sep=0.75pt]    {$r_{1}$};
% Text Node
\draw (239,253) node [anchor=north west][inner sep=0.75pt]    {$n_{2}$};
% Text Node
\draw (253,215) node [anchor=north west][inner sep=0.75pt]    {$r_{2}$};
% Text Node
\draw (300,260) node [anchor=north][inner sep=0.75pt]    {$r_{2}$};
% Text Node
\draw (337,242) node [anchor=north west][inner sep=0.75pt]    {$n_{3}$};
% Text Node
\draw (360,207) node [anchor=north west][inner sep=0.75pt]    {$r_{3}$};


==> tt-sketch.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,525); %set diagram left start at 0, and has height of 525


% ============================
% TENSOR TRAIN FORMAT
% ============================
% Text Node
%\draw (170,115) node [anchor=north][inner sep=0.75pt][align=center]{\textbf{Tensor Train (TT) Format}\\
%Grid arranged data are expressed\\
%as combination elementary tensors.};

\input{tt-blocks}

% Text Node
\draw (52,300) node [anchor=north][inner sep=0.75pt][align=center]{
$\mathcal{F}(2,1,3)\ = $};

\draw (140,300) node [anchor=north][inner sep=0.75pt][align=center] {
$\mathcal{F}^{(0)}( :,2,:)\ \cdotp $};

\draw (220,300) node [anchor=north][inner sep=0.75pt][align=center]    {
$\mathcal{F}^{(1)}( :,1,:)\ \cdotp $};

\draw (300,300) node [anchor=north][inner sep=0.75pt][align=center]    {
$\mathcal{F}^{(2)}( :,3,:)$};

% Text Node
%\draw (170,330) node [anchor=north][inner sep=0.75pt]    {$\Rightarrow %\mathcal{A}_{\mathrm{dim}}\mathcal{F}_{\mathrm{dim}} %=\mathcal{F}_{\mathrm{dim}}$};


\end{tikzpicture}

